Near-Optimal Time-Sparsity Trade-Offs for Solving Noisy Linear Equations

We present a polynomial-time reduction from solving noisy linear equations over $\mathbb{Z}/q\mathbb{Z}$ in dimension $\Theta(k\log n/\mathsf{poly}(\log k,\log q,\log\log n))$ with a uniformly random coefficient matrix to noisy linear equations over $\mathbb{Z}/q\mathbb{Z}$ in dimension $n$ where each row of the coefficient matrix has uniformly random support of size $k$. This allows us to deduce the hardness of sparse problems from their dense counterparts. In particular, we derive hardness results in the following canonical settings. 1) Assuming the $\ell$-dimensional (dense) LWE over a polynomial-size field takes time $2^{\Omega(\ell)}$, $k$-sparse LWE in dimension $n$ takes time $n^{\Omega({k}/{(\log k \cdot (\log k + \log \log n))})}.$ 2) Assuming the $\ell$-dimensional (dense) LPN over $\mathbb{F}_2$ takes time $2^{\Omega(\ell/\log \ell)}$, $k$-sparse LPN in dimension $n$ takes time $n^{\Omega(k/(\log k \cdot (\log k + \log \log n)^2))}~.$ These running time lower bounds are nearly tight as both sparse problems can be solved in time $n^{O(k)},$ given sufficiently many samples. We further give a reduction from $k$-sparse LWE to noisy tensor completion. Concretely, composing the two reductions implies that order-$k$ rank-$2^{k-1}$ noisy tensor completion in $\mathbb{R}^{n^{\otimes k}}$ takes time $n^{\Omega(k/ \log k \cdot (\log k + \log \log n))}$, assuming the exponential hardness of standard worst-case lattice problems.

==> FastNonTechnicalOverview.tex <==
We next give an overview of the proof of our main theorem, namely \cref{thm:maininformal}.
% We first focus on the case when the distribution on the support is deterministically 1.
% We show how to achieve arbitrary distribution on the support as well as varying support sizes at the end of this section.

\subsection{The High-Level Approach: Linear Mapping from Dense to Sparse Equations}%Gadget Matrices}

In what follows, we denote the input to the dense problem by $(B,y)$ and the input to the sparse problem by $(A,y')$.
Suppose we are given $(B,y)$ such that $B$ is uniform over $\mathbb{Z}_q^{m \times L}$ and we want to solve one of the decision/search/refutation problems given access to an oracle for the same problem in the sparse setting.
The high-level idea is to transform each dense equation to a sparse one in a way that preserves the approximate linear relation $b_i ^\top s\approx y$ (or absence thereof) between ``coefficients'' $b_i$ in row $i$ of $B$ and the label $y_i$.

A common approach in the literature towards this end (e.g. \cite{boneh13bit} for binary LWE, and \cite{jain24sparseLWE} for sparse LWE in certain regimes, discussed in \cref{sec:priorreduction}) is to map the coefficient vector of each equation.
If we can find a linear mapping, this will preserve the linear relation between the coefficient vector and the label.
More specifically, we aim to find a matrix $G \in \mathbb{Z}_q^{n \times L}$ (we sometime refer to this as a \emph{gadget} or \emph{decoding matrix}) such that given a sample $(b_i, y_i) \in \mathbb{Z}_q^L \times \mathbb{Z}_q$, we can efficiently find a $k$-sparse $a_i\in \mathbb{Z}_q^{n}$ such that $a_i^\top G = b_i^\top$.
Note that given this, it holds that %when $y_i \approx b_i^\top s$ for some vector $s$, this implies that $y_i \approx a_i^\top (Gs)$, that is, the approximate linear relation is preserved.
%this equation implies
\begin{align}
\label{eq:gadgeteq1}
y_i \approx b_i^\top s \text{ for some } s 
% \text{ if and only if } 
\quad \Leftrightarrow \quad y_i \approx a_i^\top (Gs) \text{ for some } s. %b_i^\top s = (a_i^\top G)s = a_i^\top (Gs).
\end{align}
Further, it should hold that the sparse equation has the correct distribution, i.e., that $a_i$ is uniform over $k$-sparse vectors in $\mathbb{Z}_q^n$.
That is, we require the following property:
\begin{align}   
\label{eq:gadgeteq2}
    \text{If }b_i\sim\unif(\mathbb{Z}_q^L), \text{ then }a_i \text{ is a uniformly random }k\text{-sparse vector in }\mathbb{Z}_q^{n}.
\end{align}


We refer to the process of computing $a$ given $b$ as the \emph{decoding algorithm}. (Indeed, a watchful reader would already have seen the analogy with syndrome decoding in coding theory).
We claim that such a primitive can imply a reduction between all of the decision/search/refutation versions.
We illustrate this here for the search task, and refer to~\cref{sec:reduction_for_all_three_tasks} for the other two tasks.\footnote{Crucially, for the refutation task we need that \emph{almost all} of the equations are mapped successfully with high probability, while this is not necessary for decision and search. See~\cref{sec:reduction_for_all_three_tasks} for details.}
Assume that $y_i = b_i^\top s + e_i$ for some error term $e_i$.
Then, we can compute the mapped equation $y_i' = y_i + a_i^\top z$, where $z \in \mathbb{Z}_q^n$ is drawn uniformly at random.
It holds that
\[
    y_i' = y_i + a_i^\top z = b_i^\top s +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i \,,
\]
where we use the same $z$ for each sample. The only role of $z$ is that the final secret $Gs + z$ is uniform over $\Z_q^n$ and independent of everything else.
Thus, given a search oracle for the sparse version we can recover $Gs + z$ and hence also $Gs$.
If $G$ is full-rank we can then recover $s$. 
%\gb{Make clear that there is a single $z$ used for all equations and that the point is to make $Gs+z$ a uniformly random secret.}


%\stefanc{additional comments gadget matrices, in particular, it should become clear already that we want $L = \omega_n(k)$}
%\kirilc{ I think this sentence is unnencessary (and wrong):
%Our main contribution is to show that such an algorithmic primitive indeed exists.}
%\stefanc{Sounds good}

%Note that an appealing property of this approach is that it preserves the error distribution.



%The quality of the reduction will depend on how large $L$ is in comparison to $n$. 
%In particular, to obtain as tight a reduction as possible, we want $L$ to be large, ideally on the order of $k \log n$.
%Since (near-)exponential hardness of the dense problem then implies (near-)$n^k$ hardness for the sparse problem.
The quality of the lower bound for the sparse problem depends crucially on the quantitative relationship between $L, n$, and $k$.
Suppose the dense problem in dimension $L$ takes time $2^{\Omega(L)}$ and that $L = f(n,k)$ for some function $f$.
Then the lower bound we can deduce for the $k$-sparse problem in dimension $n$ is $2^{\Omega(f(n,k))}$ and hence we want $f$ to grow as fast as possible.
A simple entropy argument gives a bound.
We would like vectors $b \in \mathbb{Z}_q^L,a \in \mathbb{Z}_q^n$ and a matrix $G$, such that (1) $b$ is uniform over $\mathbb{Z}_q^n$, (2) $a$ is uniform over binary $k$-sparse vectors in $\mathbb{Z}_q^n$, (3) $a^T G = b$.
Since $b$ is a function of $a$, its entropy is at most that of $a$, and this implies\footnote{In this argument we implicitly assumed that $G$ is deterministic. Since we use the same $G$ for all equations, even for a random $G$ the average entropy added on any single equation is at most $\tfrac{n L \log q}{m}$ which is negligible for all parameter settings we consider.} that $L \log q \leq k \log n$, i.e., 
\begin{equation}\label{e:entropy}
L \leq \frac{k \log n} {\log q}\,.\end{equation}
In the rest of this section, we show that this upper bound can be nearly achieved. In the most common regime of interest when $q$ is at most polynomial in the initial dimension $L,$ we also have $\log q = O(\log k + \log \log n).$  The dimension $L$ that we obtain satisfies $L = k\log n/\poly(\log k,\log\log n)$ (cf. the end of~\cref{sec:nontechnicaloverview}).
% up to lower order $\poly(\log k, \log\log n)$ factors. 
% \gb{This last sentence feels out of place unless it's connected to the prior sentence. Here's a suggestion for an alternative:}\kb{I agree. i further modified} In the rest of this section, we show that this upper bound can be nearly achieved.  (which is small in the regime that $q$ is at most polynomial in the initial dimension $L,$ in which case we obtain $\frac{k\log n}{\log q} = \frac{k\log n}{\}$). 

%\stefanc{One thing I find slightly confusing is that the entropy argument above treats $G$ as deterministic, is there a similar argument for random $G$?}
%\gb{we can make the following argument for random $G$. 1. consider all $m$ equations, 2. it's the same $G$ for all equations, and $G$ has entropy $ nL\log q$. This implies that $m L\log q\leq mk\log n + nL\log q$. So as long as $m\gg n$, essentially the same inequality holds. We could always add in a footnote saying that the randomness of $G$ makes no difference amortized over the samples.}\kb{ re: @Guy,  I am not sure I understand this comment. We never use a random $G.$ The randomness is only used to generate a $G.$ That is, if someone were to give me a deterministic ``good decoding matrix $G$' this would work just as well.}
%\gb{But you \emph{could} use a random $G$ if you wanted to, which might help make the resulting $a$ look more random to the black box. I'm just pointing out that there isn't enough randomness in $G$ to make a difference to the entropy argument.}
%\stefanc{Sounds good! I added a footnote.}

%\stefanc{This argument also shows that we only get an improvement over JLS24 if $q$ is much smaller than any polynomial in $n$. Should we state this more prominently somewhere? I think for the above argument it makes sense to add that for typical hardness assumptions $q = \poly(L)$, bc if people try to plug in $q = \poly(n)$, they might get confused. I don't really have a sense what kind of modulus you'd ideally want for the sparse variant}

%The key step in this approach is to design a gadget matrix $G\in \mathbb{Z}_q^{n\times L}$ for which the decoding step can be performed efficiently for as large $L$ as possible.

% We first describe how this enables reductions for all of decision, search, and refutation and then explain how to construct the gadget matrix and implement the decoding algorithm.





% Assuming this, the reduction works as follows:
% On input $\{(b_i,y_i)\}_{i=1}^m$, let $\{a_i\}_{i=1}^{m_1}$ be the successfully decoded $b_i$.
% If $m_1 < (1-o(1)) m$ output $\phi = 1$.
% Else, run the sparse refutation algorithm on $\{(a_i,y_i)\}_{i=1}^{m_1}$ (note that we do not change $y_i$).
% If it outputs $\phi'$ output $\phi = \phi' + o(1)$.
% Note that $\phi$ is always a correct upper bound: 1 is always an upper bound, and if $m_1 \geq (1-o(1))m$ at most a $(\phi' + o(1))$-fraction can be satisfiable.
% Else, there exists an $s$ such that $y_i = a_i^\top s$ for a larger than $\phi'$-fraction of the successfully decoded samples.
% Thus, the upper bound output by the sparse refutation algorithm cannot be correct.
% Note that with high probability $\phi$ will also be small, assuming that $\phi'$ is small with high probability (since we only output the naive upper bound 1 with probability $o(1)$).
% I.e., the strength of the refutation algorithm is preserved.

%Further, if $y_i$ was independent and uniform over $\mathbb{Z}_q$ to begin with, then so is $y_i + a_i^\top z$.
%If $y_i = b_i^\top s + e_i$, then $y_i + a_i^\top z = a_i^\top (Gs) +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i$ by \cref{eq:gadgeteq1} and $Gs + z$ is uniform over $\mathbb{Z}_q^n$.


\begin{comment}
\stefanc{The fact that the error is preserved should also imply that you can reduce between refutation problems, because the fraction of satisfied equations is preserved (up to the negligible fraction of samples you drop during the reduction)}

The high-level idea is to find some convenient gadget matrix $G\in \mathbb{Z}_q^{n\times L}$ and to solve $B = AG$ in such a way that $A$ has the correct  distribution. This is done sample by sample. That is, for each $b_i,$ one separately solves $a_i^\top G = b_i^\top.$ If one achieves this, one will be left with the following variables. $A, B = AG, y = Bs + e.$ Then, $y = AGs + e = As' + e$ where $s' = Gs$ is the new secret. A standard trick to make the new secret uniform is to draw a fresh $z\sim \unif(\mathbb{Z}_q^n)$ and add $Az$ to $y,$ thus $s_1 = s+ z\sim \unif(\mathbb{Z}_q^n).$
Hence, one obtains $(A, As_1 = e).$ The key step is to choose a gadget matrix $G$ such that one can solve $a^\top G = b^\top$ \emph{efficiently} in such a way that when $b\sim \unif(\mathbb{Z}_q^L),$ it is the case that $a$ is uniformly random $k$-sparse.
\end{comment}


\subsection{Prior Gadget Matrix Constructions and Challenges}
\label{sec:priorreduction}
The only prior work that we are aware of which reduces standard (dense) noisy linear equations to sparse ones is 
\cite{jain24sparseLWE} in the case of  \lwespace (and large-field LPN).
The authors follow the gadget matrix approach outlined above with $L = k$ and $G$ the Vandermonde matrix
\begin{align}
    G = \begin{pmatrix}
        1^0\; 1^1\; 1^2 \; \cdots\; 1^{k-1}\\
        2^0\; 2^1\; 2^2 \; \cdots\; 2^{k-1}\\
        \vdots\\
        n^0\; n^1\; n^2 \; \cdots\; n^{k-1}
    \end{pmatrix}\in \mathbb{Z}_q^{n\times k}\,.
\end{align}
To solve $a^\top G = b^\top$ on input $b\sim\unif(\mathbb{Z}_q^k)$ such that $a$ is a uniformly random $k$-sparse vector, 
they first draw a uniformly random support $S\in \binom{[n]}{k}$ \emph{independently} of $b$.
Then, they restrict $a$ and $G$ to coordinates $S$ and solve the equation $a^{\top}_SG_{S\times [k]} = b^\top$.
Whenever $q\ge n,$ \emph{every $k\times k$ minor of $G$ is of full rank} and, hence, a unique solution for $a_S$ exists.
Since $b$ is uniform over $\mathbb{Z}_q^k$, it is easy to check that $a_S$ is also uniform over $\mathbb{Z}_q^k$, so $a$ has the correct distribution.
Overall, the reduction of \cite{jain24sparseLWE} shows that $n$-dimensional $k$-sparse \lwe{} is at least as hard as $k$-dimensional \lwe; assuming exponential hardness of \lwespace implies that the $k$-sparse version takes time at least $2^{\Omega(k)}$.

We outline two ways in which one might hope to improve over this reduction:

\paragraph{Desideratum 1: Small Values of $k.$}
% As discussed before, even assuming exponential hardness of \lwe, 
As noted just above, the hardness implied by \cite{jain24sparseLWE} for $n$-dimensional \klwe{} is at best only $2^{\Omega(k)}$, which does not yield any hardness against polynomial-time (in $n$) attacks when $k = O(\log n)$. %This is a concern because certain protocols such as the linear homomorphic encryption based on sparse \lwe{} has overhead  $O(k\log \log q)$ and rate $O(k)$ and, thus, improves on previous work only in the regime $k = (\log n)^{o(1)}$ \cite{jain24sparseLWE}. The $2^{\Omega(k)}$ hardness also falls short of the conjectured $n^{\Omega(k)}$ lower bound that is frequently assumed and known to be true in restricted models of computations such as the SoS hierarchy~\cite{grigoriev2001linear,schoenebeck2008linear} and the SQ model for the related sparse \lpn problem (and, as we show, in the low-degree framework \cref{lemma:lowdegreeinzq} for sparse \lwe). 
%\gb{This paragraph is redundant and belongs in "unsatisfactory state of affairs". The only needed sentences are the first two, JLS gives $2^k$ and we need $n^k$.}
%\stefanc{I commented out the rest}
%\stefanc{I tried making the argument below a bit more concise and phrasing it in a way that ties it back in to the entropy argument we made above, here's the new version:}
It is instructive to analyze where their reduction is loose, employing a similar entropy-based argument as before.
As an intermediate step of transforming a dense $b \in \mathbb{Z}_q^L$ to a $k$-sparse $a \in \mathbb{Z}_q^n$, they compute a dense vector $\tilde{a} \in \mathbb{Z}_q^k$ such that $\tilde{a}^\top \tilde{G} = b$, for some deterministic matrix $\tilde{G}$.
Since the entropy of $\tilde{a}$ is at most $k\log q$, we must have $k \log q \geq L \log q$ and hence $L \leq k$.
Compared to the argument leading to \eqref{e:entropy}, they discard the entropy of the support of $a$ by drawing it independently from $b$.
We record this as a guiding principle:
\begin{equation}
\label{eq:P1}
\tag{P1}
\textit{
        For small $k,$ when solving $a^\top G = b^\top$, one must choose the support of $a$ based on $b$. 
    }
\end{equation}

% Stefan: previous version
\begin{comment}
\stefanc{Previous version:}
So, is there some inefficiency in the reduction of \cite{jain24sparseLWE}?
The inefficiency comes from the fact that the support $S$ 
% is not exploited because  
is drawn independently from $b$. As a simple illustration, even if one deterministically draws $S = \{1,2,\ldots, k\}$ at each step, the reduction of \cite{jain24sparseLWE} still goes through (and this makes sense since one will just obtain an instance of $k$-dimensional \lwe{} in this way). 
However, if one wants a quantitative improvement and reduce standard $L$-dimensional \lwe{} to $n$-dimensional $k$-sparse \lwe{} for some $L = \omega(k),$ the \emph{entropy of the support needs to be used}.
Indeed, note that the number of vectors $b$ over $\mathbb{Z}^L_q$ is $q^L.$
The number of $n$-dimensional $k$-sparse vectors $a$ is $\binom{n}{k}q^k$ where the $\binom{n}{k}$ contribution is from the support location and $q^k$ from the entries on the support.
If $a^\top G = b^\top$ has a solution in $a$ for any $b,$ it must be the case that $\binom{n}{k}q^k\ge q^L$ or equivalently $\binom{n}{k} \ge q^{L-k} = q^{L(1-o(1))}.$
This shows that the bulk of the entropy should come from the $\binom{n}{k}$ factor corresponding to the support location. 
\gb{this seems to only be true if $n\gg q$, no?}
\stefanc{Yes, I think this is related to my comment about $\log q$ in the previous paragraph.}
One cannot afford to lose this entropy by drawing the support independently from $b.$
We record this principle:
\begin{equation}
\label{eq:P1}
\tag{P1}
\textit{
        For small $k,$ when solving $a^\top G = b^\top$, one must choose the support of $a$ based on $b$. 
    }
\end{equation}
\end{comment}

\paragraph{Desideratum 2: Small Moduli.}
We would like our reduction to work also for small moduli, and in particular for $q = 2$ as in the case of \lpn.
Note that a key step in the reduction of \cite{jain24sparseLWE} is the inversion of an arbitrary $k \times k$ sub-matrix of $G$, which requires every $k\times k$ minor of $G$ to be full rank.
Such matrices are known as \emph{maximum distance separable} and in the regime $n\ge k,$
conjecturally, cannot exist if $q< n-2$ (e.g. \cite{huffman03fundamentals}). Hence, one cannot hope for a reduction in the important case of \lpn{} using the approach of \cite{jain24sparseLWE}.
Our approach will also rely on inverting (smaller-sized) linear systems, yet we will carefully brute-force over appropriate sub-instances and thus do not need the corresponding matrix to be full-rank.

% \paragraph{Challenge 3: Other Distributions on the Support.} Finally, it is unclear how to 
We would also like to be more versatile, e.g. obtain sparse vectors $a_i$ with distribution on the support different from uniform over $\mathbb{Z}_q^k$. As one example, our application to the hardness of tensor completion from \lwespace{} requires \emph{binary} $k$-sparse coefficients $a_i$. This does not seem possible using the approach in \cite{jain24sparseLWE}.
% , in the current work, for example, we need binary $k$-sparse samples $a_i$ for the application to tensor completion.

\subsection{A Toy Reduction for Block-wise Sparsity}

A gadget mapping dense $L$-dimensional vectors to {\em blockwise} $k$-sparse $n$-dimensional vectors is not hard to construct. A blockwise sparse vector is one whose coordinates are divided into $k$ blocks, each of which has a single non-zero coordinate. Indeed, for a parameter $t=L/k$, let $H \in \mathbb{Z}_q^{t \times q^{t}}$ denote a matrix whose columns are all the vectors in $\mathbb{Z}_q^{t}$. Then, we will let the decoding gadget $G = I_k \otimes H \in \mathbb{Z}_q^{t k \times q^{t}k}$. First of all, since $L=t k$ and $n= q^{t} k$, notice that $$ L = \frac{k\log (n/k)}{\log q} \,.$$
Secondly, given an $L$-dimensional vector $b$, one can decode each block of $t$ coordinates of $b$ into a unit vector in $q^{t}$ dimensions. Concatenating the unit vectors gives us a block-wise sparse $n$-dimensional vector $a$ such that $a^\top G = b^\top$. 
%While block-wise sparsity may suffice for some applications, we are not content with it. 

Permuting the coordinates might seem to suffice to turn blockwise sparsity into true sparsity. However, since the same permutation has to be used for all $m$ samples, the blockwise structure starts becoming apparent once one sees sufficiently many samples (we can show that $O(n^2)$ samples suffice). To decode to random sparse vectors, we need a cleverer idea which we describe next.

\subsection{Motivation for Our Reduction: Translation of Natural Languages}
We begin with a brief, completely non-rigorous overview of our implementation of the decoding procedure, motivated by how translation in the real world happens.

Our task at hand is to \emph{translate} the ``language'' of dense linear equations into the ``language'' of $k$-sparse linear equations. We take inspiration from how translation with dictionaries in the real world works. When one wants to translate a sentence from a completely unknown language, one consults the dictionary and translates it word by word. Then, one uses the grammar of the two languages to combine the individual words into statements.

In our case, the role of sentences will be taken by individual linear equations, i.e. $(b_i,y_i).$ 
We translate such a sentence by splitting the sentence $b_i$ in the dense language into words.
The grammar in the dense language is simple: a sentence of length $th$ is simply the concatenation of $t$ words of length $h.$
Then, using a dictionary, we translate each word from the dense language into a word from the sparse language, i.e., a $k$-sparse vector of smaller dimension ($\ll n$).
Finally, we use a more complicated grammar in the sparse language to piece the individual sparse words into a sparse sentence, i.e., a $k$-sparse vector in dimension $n$.
Crucially, the sparsity remains the same in this process of stitching together words, that is, we really do translate into the $k$-sparse language.

% The intuition behind efficiency of the approach is that 
The small number of possible words --- as opposed to possible sentences --- is what allows for efficient translation. Imagine if in the real world one had to print a dictionary containing 
translations of all possible sentences!
Our key contribution is constructing the ``grammar'' of sparse equations, i.e., the rules for how to combine multiple $k$-sparse vectors in a smaller dimension into a $k$-sparse vector in a larger dimension.
This is necessary, because simply concatenating them would blow-up the sparsity by a multiplicative factor of the number of words, which would be too large.

% \gb{I think we need to convey a bit more what is the "magic" here. Why is it non obvious that decomposition like this can work?}
% \stefanc{I think the key point is that the sparsity for the ``sparse words'' and the ``sparse sentences'' is the same, i.e., the first are $k$-sparse vectors over a small dimension and the second are also $k$-sparse (for the same $k$), but over a larger dimension.}\kirilc{I really like this section as it is right now. To me, its purpose is that readers will be ``ahaa, this is actually very simple and I can read the math that follows it.''}

\subsection{Overview of Our Reduction to Sparse Equations} 
\label{sec:nontechnicaloverview}
We begin by explaining the reduction in the case that the distribution on the support is deterministically equal to 1, which captures both sparse problems \klpn{} and \emph{binary} \klwe.
At the end of this section, we explain how a simple modification addresses arbitrary distributions on the support.

\stefanc{Maybe we can move an abridged version to earlier in the section?}
%We start with the same idea as in \cite{jain24sparseLWE}.
Recall that as in~\cite{jain24sparseLWE}, we want to construct a gadget matrix $G\in \mathbb{Z}_q^{n\times L}$ and, on input a uniform random $b \in \mathbb{Z}_q^L$, solve $a^\top G = b^\top$ for a $k$-sparse $a\in \{0,1\}^n$. 
However, as observed in \eqref{eq:P1}, in doing so, we need to use the randomness of $b$ in choosing the location of the support of $a.$
In particular, we need to sample from (some large enough subset of) the possible supports. This task can be interpreted as a sampling version of 
the popular $k$-SUM problem, in which given $n$ vectors  in $\mathbb{Z}_q^L$ and a target $b$ one needs to find $k$ of them that sum to $b.$
Evidence for hardness of this problem exists both in the average-case setting (when 
the $n$ vectors are random)
based on lattice problems \cite{brakerski2020hardness} and in the setting of worst-case vectors based on the exponential-time hypothesis \cite{patrascu10fastersat,abboud22sethksum}. Essentially, these results state that the time required is $\min(n^k, 2^{L/\log k})$, both of which are too slow for our purposes. Instead, we need a reduction that runs in time $n^{o(k)}$ (to conclude $n^{o(k)}$ hardness of $k$-sparse \lwe) and $2^{L/\log L} = 2^{L/\log \omega(k)}$ in the relevant regime $L = \omega(k)$
in the case of \lpn{} (as our reduction needs to be faster than the strongest plausible $2^{L/\log L}$ hardness of \lpn). This step of solving $k$-sum poses a serious obstacle to our approach. Unfortunately,
our task is actually even harder -- we furthermore need to \emph{sample} from the $k$-SUM solutions. 

We circumvent the hardness of $k$-sum by endowing $G$ with a convenient structure that makes finding solutions and sampling from them easy.

\paragraph{Representing Uniformly Sparse Solutions as Steps of Random Walks.}

Consider for a moment the reverse direction of what we are trying to show.
I.e., given a uniformly random $k$-sparse vector $a$ in dimension $n$, design a matrix $G$, such that the distribution $b = a^\top G \in \mathbb{Z}_q^L$ is (close to) the uniform distribution over dense vectors.
Note that, thinking of the entries of $a$ as a $k$-tuple with repetitions allowed, this has a natural interpretation as the following random process:
Start with the all-zeroes vector and for $k$ steps, choose a row of $G$ at random and add it to the current state.
In particular, we can think of the steps of the random walk, i.e., the entries of the $k$-tuple, as an implicit representation of $b$ (together with the gadget matrix $G$).
The task of finding a good gadget matrix $G$ is now a task of designing update rules of a random walk such that the walk mixes quickly.

Taking this viewpoint, it becomes clear that \emph{redundancy} (in terms of the number of steps we take) is key to achieve uniformity of the final state/vector.
In particular, the most canonical random walk over $\mathbb{Z}_q^L$ is as follows: at every step, choose a random coordinate and add a uniformly random element over $\mathbb{Z}_q$ to it.
As we will see, this also has a very natural encoding as a gadget matrix $G$.
This walk converges to an almost uniform state in roughly $L (\log L + \log q)$ steps.
Conversely, we could hope that the reverse direction is also true, i.e., given a uniform vector $b$, its implicit representation in terms of steps of this walk is close to uniform over all $k$-tuples, as long as $k \approx L \log L$.
We could then try to decode this $k$-tuple into a $k$-sparse vector.

Even assuming uniformity of this implicit representation, and that we can efficiently find one, this has the obvious drawback that the size of the representation is even larger than the initial dimension.
And thus, we will likely not be able to decode it into a sparse vector (where the sparsity is supposed to be much smaller than the dimension).
However, one of our main insights is that that this line of reasoning still applies to sub-strings of the input $b$.\footnote{The idea to split the problem into smaller sub-problems is similar to the celebrated BKW algorithm \cite{BKW}.}
In particular, writing $b = (b_1, \ldots, b_t)$, our reduction rests on the following two properties:
\begin{enumerate}
    \item Given a uniform $b_i \in \Z_q^{h}$, we can efficiently compute an implicit representation of $b_i$ that is (close to) uniform over all $k$-tuples (over some small domain) such that $k \approx h (\log h + \log q) \ll n$.
    \item We can efficiently combine all implicit representations of the $b_i$ to a representation of $b$ as a $k$-tuple over $[n]$.
    Further, if all initial representations are uniform, the final one will be as well.
\end{enumerate}
Crucially, the size of the representation does not increase in the last step (only the size of the domain).
We can easily decode the final $k$-tuple into a $k$-sparse vector.


\paragraph{Word Decoding: Finding Uniform Implicit Representations of Small Sub-Problems}

More formally, we represent each $b\in \mathbb{Z}_q^L$ as $(b_{1}, b_{2}, \ldots, b_{t})$, where each $b_i \in \mathbb{Z}_q^h$.
% We will think of each $b_i$ as a concatenation of $t$ independent strings  of length $h.$ 
We will decode each $b_{j}$ into a $k$-tuple of indices over $[hq]^k$ via a smaller gadget matrix $V \in \mathbb{Z}_q^{hq \times h}$ (this is the dictionary mentioned above).
The following gadget matrix corresponds to the lazy random walk over $\mathbb{Z}_q^h$.
%As we will need to solve $k$-SUM over this $V,$ it is natural that we want $V$ to have a very simple explicit structure. We take $V$ to contain all multiples of the identity:
\begin{align*}
    V= 
    \begin{pmatrix}
      0 \times I_h\\
      1\times I_h\\
      \quad \vdots\\
      (q-1)\times I_h
    \end{pmatrix}.
\end{align*}
We call the $hq$ rows $V_{1,:}, V_{2,:},\ldots, V_{hq,:} \in \mathbb{Z}^h_q$ words.
%Here, $h$ is the word length.
We want to find $\xi_j = (\xi_j(1),  \ldots, \xi_j(k)) \in [hq]^k$ such that the sum of the rows of $V$ indexed by $\xi_j$ is equal to $b_j$ %$$\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}\,.$$ % (hereon, we identify $k$-sparse binary vectors with $k$-tuples of indices). 
Furthermore, if $b_j$ is uniform over $\mathbb{Z}_q^h$, we will require the marginal distribution of $\xi_j$ to be uniform over $[hq]^k$.
In particular, consider the set of all such $\xi_j$
\begin{equation}
\label{eq:preimagedef}
\begin{split}
\Preimage_{V}(b) \coloneqq \Set{(\xi(1), \xi(2), \ldots,\xi(k))\in [hq]^k\suchthat \sum_{\psi = 1}^k V_{\xi(\psi).:} = b}.
\end{split}
\end{equation}
We will show that (1), we can efficiently sample a uniform element from $\Preimage_{V}(b)$ and (2), for a uniformly random $b$, this is close to uniform over all $k$-tuples.
We can make the distribution exactly uniform by a simple rejection sampling step.

Towards (1) we show the following lemma.
\begin{lemma}[Efficient preimage sampling]
\label{lem:samplingintro}
% There exists an algorithm (\cref{alg:samplingfrompreimage}) with the following property.
On input $k>h+2$ and $b \in \mathbb{Z}_q^h,$ there exists an algorithm (cf.~\cref{alg:samplingfrompreimage}) that outputs a uniformly random element of $\Preimage_V(b).$ The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}
On a high level, this can (roughly) be achieved by sampling indices uniformly at random (from $[hq]$) until the number of indices left matches the number of coordinates that differ between the current state and $b$.
The choice of the remaining coordinates is then fixed.
Permuting them randomly will result in a uniformly random element from the preimage.

%When combining the different words into sentences, a key property will be that $\xi_j(1),  \ldots, \xi_j(k)$ are (nearly) independent and uniform over $[hq].$ To guarantee this, a key property will be that each $\Preimage_V(b)$ is of nearly equal size. Otherwise, $k$-tuples $\xi_j(1),  \ldots, \xi_j(k)$ corresponding to $b$ with large (respectively, small)
%$\Preimage_V(b)$ will be under-represented (respectively, over-represented). Again, the simple structure of $V$ can be utilized to show the following fact.
Note that the sets $\Preimage_{V}(b)$ partition the set of all $k$-tuples over $[hq]^k$.
Thus, if all of these parts have (roughly) the same size, outputting a random element from one of them will be close to uniformly random (on input a uniformly random $b$).
More specifically, we show the following.
\begin{lemma}[Uniformity of preimage size]
\label{lem:nearuniformityintro}
    Suppose that $k \ge 4h(\log h +\log q +  \log (1/\psi))$ where $\psi\in (0,1)$ is any real number. Then, for each $u \in \mathbb{Z}_q^h$,
    $$
    \frac{(1-\psi)(hq)^k}{q^h}\le 
    |\Preimage_V(u)|
    \le 
    \frac{(1+\psi)(hq)^k}{q^h}.
    $$
\end{lemma}
We give the proof in \cref{sec:randomwalkproof}, which follows by analyzing the point-wise convergence of the lazy random walk on $\mathbb{Z}_q^h$. Note that it is well-known that this walk converges to the uniform distribution in total variation distance after roughly $h (\log h + \log q)$ steps. For our applications, the stronger, point-wise converges guarantee is crucial.
In particular, trying to deduce a point-wise converge bound from the total variation bound would require $k \gtrsim h^2$ which would result in a much looser lower bound.
% 
For reasons that will become clear, we will choose $\psi = o(1/t),$ say $\psi = (ht)^{-2}.$

In order to make the output tuples exactly uniform, we will use a simple rejection-based method that rejects each $b_j$ with probability $$1 - \frac{|\Preimage_V(b_j)|}{{(1+\psi)(hq)^k}/{q^h}},$$ which is a well-defined probability and is at most 
$2\psi$ under the guarantee of \cref{lem:nearuniformityintro}.
To make this algorithmically efficient, we need to be able to compute $|\Preimage_V(b_j)|.$
This will follow by first observing that by symmetry considerations, the size of the set only depends on the number of non-zero entries of $b_j$.
Then, the size can be efficiently computed via dynamic programming.
\begin{lemma}[Computing preimage size]
\label{lem:sizeestimationintro}
There exists an algorithm (cf.~\cref{alg:sizeestimation}) that on input $k$ and $b \in \mathbb{Z}_q^h,$ outputs
$|\Preimage_V(b)|.$
The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}

% Stefan: Previous Version
\begin{comment}
\paragraph{Word Decoding: Splitting into Small Sub-Problems That Can Be Solved Efficiently.}
We will decompose the problem into $t$ sub-problems by splitting the string $b$ into $t$ equal parts (similar to the celebrated BKW algorithm \cite{BKW}).
These parts of size $h\coloneqq L/t$ will be small enough that we can efficiently find a representation using $k$-tuples in each part, and these will then be carefully combined.
%Then, we will combine these $t$ small sub-problems.
It will be convenient to work with $k$-tuples of indices for now, i.e., allow repeated indices. We will be able to show that only a negligible fraction actually has repeated indices, so that we can represent most of them as $k$-sparse vectors.
% \stefanc{I would mention that again we need sth like $r^k \geq 2^(L/t)$ -> need $t$ not too small}

More formally, represent each $b\in \mathbb{Z}_q^L$ as a concatenation of $t$ uniform independent strings $b = (b_{1}, b_{2}, \ldots, b_{t})$ in $\mathbb{Z}_q^h$.
% We will think of each $b_i$ as a concatenation of $t$ independent strings  of length $h.$ 
We will decode each $b_{j}$ into a $k$-tuple of indices over $[hq]^k$ via a smaller gadget matrix $V \in \mathbb{Z}_q^{hq \times h}$ (this is the dictionary mentioned above). As we will need to solve $k$-SUM over this $V,$ it is natural that we want $V$ to have a very simple explicit structure. We take $V$ to contain all multiples of the identity:
\begin{align*}
    V= 
    \begin{pmatrix}
      0 \times I_h\\
      1\times I_h\\
      \quad \vdots\\
      (q-1)\times I_h
    \end{pmatrix}.
\end{align*}
We call the $hq$ rows $V_{1,:}, V_{2,:},\ldots, V_{hq,:} \in \mathbb{Z}^h_q$ words.
%Here, $h$ is the word length.
We want to find $\xi_j = (\xi_j(1),  \ldots, \xi_j(k)) \in [hq]^k$ such that $$\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}\,.$$ % (hereon, we identify $k$-sparse binary vectors with $k$-tuples of indices). 
Furthermore, if $b_j$ is uniform over $\mathbb{Z}_q^h$, we will require the marginal distribution of $\xi_j$ to be uniform over $[hq]^k$.
We achieve this by outputting a uniformly random $\xi_j$ that satisfies $\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}$.

Here, we take the opportunity to introduce some useful notation:
\begin{equation}
\label{eq:preimagedef}
\begin{split}
\Preimage_{V}(b) \coloneqq \Set{(\xi(1), \xi(2), \ldots,\xi(k))\in [hq]^k\suchthat \sum_{\psi = 1}^k V_{\xi(\psi).:} = b}.
\end{split}
\end{equation}
The simple structure of $V$ allows for extremely efficient sampling from the preimage of $b.$

\begin{lemma}[Efficient preimage sampling]
\label{lem:samplingintro}
% There exists an algorithm (\cref{alg:samplingfrompreimage}) with the following property.
On input $k>h+2$ and $b \in \mathbb{Z}_q^h,$ \cref{alg:samplingfrompreimage} outputs a uniformly random sample from $\Preimage_V(b).$ The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}

When combining the different words into sentences, a key property will be that $\xi_j(1),  \ldots, \xi_j(k)$ are (nearly) independent and uniform over $[hq].$ To guarantee this, a key property will be that each $\Preimage_V(b)$ is of nearly equal size. Otherwise, $k$-tuples $\xi_j(1),  \ldots, \xi_j(k)$ corresponding to $b$ with large (respectively, small)
$\Preimage_V(b)$ will be under-represented (respectively, over-represented). Again, the simple structure of $V$ can be utilized to show the following fact.

\begin{lemma}[Uniformity of preimage size]
\label{lem:nearuniformityintro}
    Suppose that $k \ge 4h(\log h +\log q +  \log (1/\psi))$ where $\psi\in (0,1)$ is any real number. Then, for each $u \in \mathbb{Z}_q^h$,
    $$
    \frac{(1-\psi)(hq)^k}{q^h}\le 
    |\Preimage_V(u)|
    \le 
    \frac{(1+\psi)(hq)^k}{q^h}.
    $$
\end{lemma}
We give the proof in \cref{sec:randomwalkproof}, which follows by analyzing the point-wise convergence to the uniform distribution of a naturally occurring Markov chain over $\mathbb{Z}_q^h$.
% 
For reasons that will become clear, we will choose $\psi = o(1/t),$ say $\psi = (ht)^{-2}.$

In order to make the output tuples exactly equal, we will use a simple rejection-based method that rejects each $b_j$ with probability $$1 - \frac{|\Preimage_V(b_j)|}{{(1+\psi)(hq)^k}/{q^h}},$$ which is a well-defined probability and is at most 
$2\psi$ under the guarantee of \cref{lem:nearuniformityintro}.
To make this algorithmically efficient, we need to be able to compute $|\Preimage_V(b_j)|.$ Again, the simple structure of $V$ allows such a primitive:

\begin{lemma}[Computing preimage size]
\label{lem:sizeestimationintro}
There exists an algorithm, \cref{alg:sizeestimation}, which on input $k$ and $b \in \mathbb{Z}_q^h,$ outputs
$|\Preimage_V(b)|.$
The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}
\end{comment}

\paragraph{Sentence Decoding: Combining the Solutions of Small Sub-Problems.}
 We will think of concatenations of words as sentences.
 Each sentence will have exactly $t$ words.
 The rows of our final gadget matrix will be all possible sentences, of which there are $ (hq)^t$.

Let $n = (hq)^t$.
We will use the decodings $\{\xi_j\}_{j=1}^t$ of $\{b_{j}\}_{j = 1}^t$ obtained via the matrix $V$ to produce a $k$-tuple $\xi \in [n]^k = ([hq]^t)^k$ decoding of $b.$ The key insight is that $\{b_{j}\}_{j = 1}^t$ are $t$ iid vectors in $\Z_q^h$ and, hence, $\{\xi_j\}_{j=1}^t$ are $t$ iid tuples in $[hq]^k.$ In particular, $(\xi_j(\psi))_{1\le j \le t, 1\le \psi\le k}$ are $kt$ independent uniform integers in $[hq].$

By definition, $\xi$ should be uniformly random. We define $\xi(\psi)\coloneqq (\xi_1(\psi),\xi_2(\psi),\ldots, \xi_t(\psi))$ for $1 \leq \psi \leq k$ and $\xi= (\xi(1), \xi(2), \ldots, \xi(k)).$ Visually, we represent $\xi$ as the following matrix in $[hq]^{t\times k}.$
$$\xi = 
\begin{pmatrix}
    \xi_1(1) \; \xi_1(2)\; \ldots \; \xi_1(k)\\
    \xi_2(1) \; \xi_2(2) \; \ldots\; \xi_2(k)\\
    \vdots\\
    \xi_t(1)\; \xi_t(2)\; \ldots  \; \xi_t(k)\\
\end{pmatrix}.
$$
In it, each row corresponds to a decoded word (that is, $\xi_j(1), \xi_j(2), \ldots, \xi_j(k)$ is the $k$-tuple corresponding to $b_j$). Each column $\xi(\psi) = (\xi_1(\psi), \xi_2(\psi), \ldots, \xi_t(\psi))^\top$ corresponds to a $t$-tuple in $[hq]^t$ and, hence, can be treated as an index in $[(hq)^t] = [n].$ This is the $k$-sparse grammar we referred to.
Crucially, each of the $k$ indices (columns) are independent uniform. Thus, we have managed to translate $b\in \Z_q^{ht}$ into $k$ uniform independent indices in $[(hq)^t] = [n],$ as desired. 

To finish, we put this in the language of gadget matrices and demonstrate a linear relationship between $b$ and $\xi.$ Let $G\in \mathbb{Z}_q^{n \times L}$ be such that its rows are indexed by $ (\phi_1, \ldots, \phi_t) \in [hq]^t$ and each row is defined by
\begin{equation}
\label{eq:gdefintro}
G_{(\phi_1, \phi_2,\ldots, \phi_t),:} = 
(V_{\phi_1,:},V_{\phi_2,:},\ldots, V_{\phi_t,:})\in \mathbb{Z}_q^{ht} = \mathbb{Z}_q^{L} \,.
\end{equation} 
In other words, $G$ contains all possible concatenations of $t$ words from $V.$
%We think of each $t$-tuple of words from $W$ as a sentence and, hence, $G$ consists of all possible sentences using $t$ words.
% We offer the following illustration for $t = 3$, where $\mathbbm{1}_r$ is the all-ones vector in $\mathbb{R}^r$
% \[\arraycolsep=8pt
% G(W) = \left(\begin{array}{ccc}
% w_1^\top \otimes \mathbbm{1}_r & w_1^\top \otimes \mathbbm{1}_r & W \\
% \vdots & \vdots & \vdots \\
% w_1^\top \otimes \mathbbm{1}_r & w_r^\top \otimes \mathbbm{1}_r & W \\
% \\
% \hline 
% \\
% \vdots & \vdots & \vdots \\
% \\
% \hline \\
% w_r^\top \otimes \mathbbm{1}_r & w_1^\top \otimes \mathbbm{1}_r & W \\
% \vdots & \vdots & \vdots \\
% w_r^\top \otimes \mathbbm{1}_r & w_r^\top \otimes \mathbbm{1}_r & W \\
% \end{array} \right)\,.
% \]



Since $\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}^\top$ holds for each $j$, it must be the case that 
\begin{equation}
\begin{split}
\label{eq:introsumingadget}
\sum_{\psi = 1}^k G_{\xi(\psi)} &= \sum_{\psi = 1}^k
 \Big( V_{\xi_1(\psi),:},V_{\xi_2(\psi),:},\ldots, V_{\xi_t(\psi),:}\Big) = \bigg( \sum_{\psi = 1}^k V_{\xi_1(\psi),:},  \sum_{\psi = 1}^k V_{\xi_2(\psi),:},\ldots,  \sum_{\psi = 1}^k V_{\xi_t(\psi),:}\bigg) \\
 &= \big( b_1^\top, b_2^\top, \ldots, b_t^\top\big) = b^\top\,.
 \end{split}
\end{equation}
Under a mild condition $k = o(\sqrt{n}),$ the birthday paradox shows that with high probability, all of the $\xi(\psi)$ are distinct. When this event holds we can represent $\xi$ as a (binary) $k$-sparse vector $a$ that is uniformly random (the non-zero coordinates of $a$ are indexed by $\xi(1), \xi(2), \ldots, \xi(k)$).
\eqref{eq:introsumingadget} is equivalent to $a^\top G = b^\top$ as desired.

%Ignoring the fact that there might exist $\psi_1\neq \psi_2$ such that $\xi(\psi_1) = \xi(\psi_2),$ we are left with uniform $k$-tuples over $G.$ Hence if $a \in \mathbb{Z}_q^n = \mathbb{Z}_q^{r^t}$ is such that $a(\xi(\psi)) = 1$ for all $\psi \in \{1,2,\ldots, k\}$ and $a(\zeta) = 0$ otherwise, we are left with a $k$-sparse vector $a$ such that $a^\top G = b^\top.$

% Stefan: Most of this is in the paragraph in the beginning, so we could remove this
\begin{comment}
\paragraph{Endgame.}
Altogether, we have $AG(W) = B$ and the matrix $A$ is drawn uniformly from the binary $k$-sparse  \lwe. Hence, we transform $(B, Bs + e)$ into $(A, AG(W)s + e).$ We are not done yet as the secret $Gs$ is not uniform over $\mathbb{Z}_q^{n}$ as it is in the column span of $G \in \mathbb{Z}_q^{n\times L}$ which is clearly not full rank ($L\ll n$). Nevertheless, we can simply choose a fresh $z\sim \mathbb{Z}_q^n$ and find $(A, A(Gs+z) + e).$  Now, $s_1 = Gs + z\sim \unif(\mathbb{Z}_q^n).$ 
 
This concludes the reduction for the decision problem in the case $\mathcal{D}\equiv 1^k.$ When reducing between the search and refutation problems, some extra steps are needed but these are mostly technical details. In particular, for search we require that $G$ is of rank $L$ and for refutation that even for worst case $b_j,$ the $k$-tuple $\xi_j(1), \xi_j(2), \ldots, \xi_j(k)$ consists of pairwise different indices with high probability.
\end{comment}

\paragraph{Other Distributions on the Support.} 
Given a vector $b\in \mathbb{Z}_q^L,$ we first solve the binary problem. That is, find a $k$-tuple $(i_1, \ldots, i_k) \in [n]^k$ such that the corresponding rows of $G$ sum to $b$.
If $b$ is uniform, then so is $(i_1, \ldots, i_k),$ as already mentioned.
%For each sample $b,$ we use the sentence-decoding matrix $G(V)$ to find some $k$-sparse binary $a$ such that $a^\top G(V) = b^\top$ whose support is furthermore uniformly distributed. Let the support be $(i_1, i_2, \ldots, i_k)\in [n]^k.$
Next, sample $\rho = (\rho_1, \rho_2, \ldots, \rho_k)\in (\mathbb{Z}_q\backslash\{0\})^k$ from $\mathcal{D}$.
Suppose that the row of $G$ indexed by $i_j$ corresponds to
\[
(\kappa_1(j)e^\top_{\Delta_1(j)},\kappa_2(j)e^\top_{\Delta_2(j)},\ldots, \kappa_t(j)e^\top_{\Delta_t(j)}) \,,
\]
where $\kappa_i(j) \in 
\mathbb{Z}_q$ and $\Delta_i(j) \in [h].$
We use the convention that the first $h$ (zero) rows of $V$ are $0e_1^\top,0e_2^\top,\ldots,0e_s^\top.$
Now, replace this index with the index $i_j'$ corresponding to
\[
(\kappa_1(j)\rho_j^{-1}e^\top_{\Delta_1(j)},\kappa_2(j)\rho_j^{-1}e^\top_{\Delta_2(j)},\ldots, \kappa_t(j)\rho_j^{-1}e^\top_{\Delta_t(j)})\,.
\]
Since $\rho_j \neq 0$, $i_j'$ is still uniform over $[n]$.
Suppose again that all $i_j'$ are distinct, we can show that this happens with high probability.
Let $a'$ be the vector with support $(i'_1, i'_2, \ldots, i'_k)$ such that $a'_{i'_j} = \rho_j$.
Then, $(a')^\top G = a^\top G = b^\top$ and clearly the support of $a'$ is uniform and the distribution on the support equal to $\cD$.

\paragraph{Variable Support Sizes.} Finally, we can also accommodate for varying support sizes. The reason is that all of our primitives - \cref{lem:samplingintro,lem:sizeestimationintro,lem:nearuniformityintro} only rely on $k$ being sufficiently large and, thus, it is enough to accommodate for the effectively smallest possible support size $k.$

More concretely,
suppose that the distribution of support sizes is $\mathcal{K}$ where with probability $1 - \eta$ with $\eta = o(1/m)$ the support size is at least $k_\minsf.$ Then, for each sample $b_i,$ we first draw $k_i\sim \mathcal{K}$ and then use the word-decoding and sentence-decoding procedures for $k_i.$
We can show that the $k$-tuples are still uniform for all $k_i \ge k_\minsf$ if the input $b$ is random.
With high probability, we never see $k_i< k_\minsf.$ More detail is given in \cref{sec:variablesupportsizes}.


\paragraph{Summary of Parameters.} We summarize the parameters for convenience of the reader.

\begin{equation}
\label{eq:parameters}
\begin{split}
& \textsf{PROBLEM PARAMETERS:}\\
& \quad\quad\quad k \text{ sparsity},\\
& \quad\quad\quad n \text{ target dimension},\\
& \quad\quad\quad L \text{ initial dimension},\\
& \quad\quad\quad q \text{ modulus}.\\
& \textsf{AUXILIARY PARAMETERS FOR REDUCTION:}\\
& \quad\quad\quad hq \text{ number of words in } V,\\
& \quad\quad\quad h \text{ word length in } V,\\
& \quad\quad\quad t \text{ sentence length}.\\
& \textsf{RELATIONSHIPS:}\\
& \quad\quad\quad n = (hq)^t\Longleftrightarrow t = \frac{\log n}{\log h + \log q},\\
& \quad\quad\quad L = ht\Longleftrightarrow  L =  \frac{h \log n}{\log h + \log q}\\
& \quad\quad\quad k \ge 4h(\log h + \log q + 2\log ht)
\end{split}
\end{equation}

\paragraph{Example Choice of Parameters for LPN.} The running time of our reduction is \linebreak $\poly(n,m,h,k) = \poly(n,m).$
In order to obtain hardness results, we need to ensure that this $\poly(n,m)$ running time is less than the assumed hardness of the initial $L$-dimensional noisy linear equation problem.
We formally choose the parameters in \cref{sec:parameters} but here we give a brief intuition about how large they are for concreteness.
For simplicity, we focus on the decision version of \lpn, i.e., $q = 2$.
We assume $2^{\Omega(L/\log L)}$ hardness of standard  \lpn{} and will derive a $n^{\Omega(\frac{k}{\log k (\log k + \log \log n)^2})}$ lower bound for the $k$-sparse decision version for suitable $k.$

Note that $t = \frac{\log n}{\log h + \log q} = \frac{\log n}{1 + \log h}.$ Hence, $L = ht = \frac{h\log n}{1 + \log h}.$ This value is clearly increasing in $h.$ Thus, we want to choose the largest $h$ possible.

Note, however that 
$k \ge 4h(\log h + \log q + \log (ht)^2)$ and $4h(\log h + \log q + \log (ht)^2) = \Theta(h(\log h + \log\log n)).$ Hence, we can choose $h$ at most $h = C\frac{k}{\log k + \log\log n}$ for some small absolute constant $C>0.$ Thus, $t = \frac{\log n}{\log h + \log q} =\Theta(\frac{\log n}{\log k}).$ 

Altogether, $L = ht = \Theta(\frac{k\log n}{\log k(\log k + \log\log n)}).$ We obtain  $$\exp\Big(\Omega\big(\frac{L}{\log L}\big)\Big) = \exp\Big(\Omega\big(\frac{k\log n}{\log k(\log k + \log\log n)^2}\big)\Big)$$ hardness.

% Sparse LPN:
% \begin{enumerate}
%     \item Sparse \lpn introduced by \cite{alekhovich03averagecasevsapproximation}
%     \item Some hardness evidence: \cite{liu17hardnesssparselpn}. Either sparse \lpn is hard or can build PKE from it.
%     \item 
%     \item \emph{Statistics:} \cite{feige02refutingkxor}, hardness of refuting random $k$-xor. And, \cite{Allen2015HowTR,barak16noisytensor,raghavendra17stronglyrefuting} refutation algorithms and SoS lower bounds.
%     \item \emph{Statistics:} \kirilc{Stefan, I think at some point of time you said something about hardness of learning halfspaces. Were you referring to the paper "Complexity theoretic limitations on learning DNF’s"?}
%     \item \emph{Crypto:} \cite{applebaum10pkcryptographyfromdifferentasssumptions} public-key crypto; Related to [NikonSeyoonVinod24] IO; Multiparty Homomorphic Secret Sharing (HSS) --- Jain, Lin et al.; Pseudorandom Correlation Generators.
    
%     \item \emph{Some variants and cousins:} 
%     \cite{dao24sparsedense} sparse-dense  \lpn.
% \end{enumerate}
% \medskip

% Sparse LWE: [A systematic Study of Sparse LWE, Aayush Jain Huijia Lin Sagnik Saha].

% \medskip

% Yet, very little known in terms of reductions. This is our main contribution.




% To formally state our result, for any $1\le m_1\le m,$ denote by $\mathcal{E}_{m_1}$ the distribution formed drawing $X\in \mathbb{Z}^m_q$ from $\mathcal{E}$ and restricting $X$ to a uniformly random subset of $m_1$ coordinates. Note that when $\mathcal{E}$ is the $m$-fold product distribution $\mathcal{F}^{\otimes m},$ then $\mathcal{E}_{m_1} = \mathcal{F}^{\otimes m_1}.$








\subsection{Reduction for Decision, Search, and Refutation}
\label{sec:reduction_for_all_three_tasks}

As before, \cref{eq:gadgeteq1,eq:gadgeteq2} are sufficient to obtain a reduction for any of the decision, search, and refutation tasks.
%Indeed, this is easiest to see for the search task.
%Assume that $y_i = b_i^\top s + e_i$ for some error term $e_i$.
%Then, on input $\{(b_i, y_i)\}_{i=1}^m$, we can compute $\{a_i\}_{i=1}^m$ as above and output $\{(a_i, y_i' \coloneqq y_i + a_i^\top z)\}$, where $z \in \mathbb{Z}_q^n$ is drawn uniformly at random (we add $a_i^\top z$ so that the secret is uniformly random).
%Note that $a_i$ has the correct distribution by \cref{eq:gadgeteq2}.
%Further, it holds that
%\[
%    y_i' = y_i + a_i^\top z = a_i^\top (Gs) +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i \,,
%\]
%where $Gs + z$ is uniform over $\mathbb{Z}_q^n$.
Thus, given a search oracle we can recover $Gs + z$ and hence also $Gs$.
%Under the additional assumption that $G$ is full-rank we can then recover $s$.
%Our construction will have this property.
We already discussed this for the search task.
Recall that given $(b_i, y_i)$, our reduction outputs $(a_i, y_i' \coloneqq y_i + a_i^\top z)$, where $z$ is uniform over $\mathbb{Z}_q^n$.
Note that this implies that the ``planted'' distribution of the decision task will be mapped correctly.
Similarly, if in the original input $y_i$ and $b_i$ are independent then so will $y_i'$ and $a_i$ be since decoding $b_i$ into $a_i$ does not depend on $y_i$ and $y_i' = a_i^\top z + y_i$.
Note that for both decision and search, the reduction preserves the error of each equation.

% \stefanc{ToDo: Check if notation is consistent with preliniaries and technical sections}\kirilc{I think we need to fix notation here, but otherwise I really like this paragraph!}
Lastly, we discuss refutation. For simplicity of exposition, we focus on the \lpn{} setting here, but the same arguments apply to \lwe{} (see \cref{sec:reductionandtasks}).
% In particular, given $(A,y)$ we want to output a value $\phi \in [0,1]$ such that at most a $\phi$-fraction of the equations $(A,y)$ are satisfiable simultaneously.\footnote{We can also handle more general refutation tasks with respect to other error metrics, see~\cref{sec:tasks}.}
% % Further, with high probability $\phi$ should be small (ideally close to 1/2, since that is the tightest upper bound with high probability).
% % In the above we considered the slightly idealized setting in which every equation is decoded successfully with probability 1.
% % Note that for decision and search even only preserving a small 1/100 (or less) fraction of the samples would be sufficient.
% % For refutation, this is not sufficient, since our algorithm has to produce a correct upper bound on \emph{all} inputs.
% % An extreme case would be when the input is highly satisfiable, e.g., due to many duplicate rows, and the decoding process looses all the equations that make it highly satisfiable.
% % Luckily, we are able to construct gadget matrices and a decoding algorithm that only loose an $o(1)$-fraction of the samples.
Given $(A,y),$ we want two guarantees. For all approximately-satisfiable systems, i.e. $As\approx y$ for some $s,$ we want to output \textit{approximately satisfiable} with probability 1.
For the case when $A,y$ are drawn independently (and hence the system is far from satisfiable with high probability), we want to output \textit{strongly unsatisfiable}, with high probability.
% In the above we considered the slightly idealized setting in which every equation is decoded successfully with probability 1.

In the discussion on search and testing, we considered the slightly idealized setting in which every equation is decoded successfully. Yet, many reductions (including ours) lose samples.
Note that for decision and search even only preserving a small 1/100 (or less) fraction of the samples would be sufficient.
For refutation, this is not sufficient since our algorithm has to map approximately satisfiable inputs to approximately satisfiable outputs. Yet, consider the following extreme case. A very large $99/100$ fraction of the clauses in the input are satisfiable due to the fact that they are all the same $(a_1,y_1).$ The rest $1/100$ of instances are highly unsatisfiable. 
A decoding process which always fails on $a_1$ and succeeds on all the other samples
would lose the $99/100$ fraction of satisfiable equations and
could produce a highly unsatisfiable instance. 

Luckily, we are able to construct gadget matrices and a decoding algorithm that only lose a $o(1)$-fraction of the samples with high probability over worst-case inputs. Indeed, recall that each $b_j\in \Z_q^h$ is rejected with probability at most $O(\psi) = O((ht)^{-2})$ and, hence, $b$ is rejected with probability at most $O(t(ht)^{-2}) = o(1).$
This resolves the above-described issue. Hence, our reduction maps approximately satisfiable instances to approximately satisfiable instances and instances with $B,y$ independent to instances with $A,y$ independent. 
Thus, it also works for refutation.



\subsection{Organization of the Rest of the Paper}
In \cref{sec:background_short} we give formal definitions and summarize relevant prior work.
In \cref{sec:ourcontributions} we formally state our results.
%Then, we explain the challenges in reducing dense linear equations to sparse linear equations and overview how we overcome these challenges.
The following section \cref{sec:reductiontosparsity} contains the full reduction.
Our reduction as well as its run-time are parametrized. In \cref{sec:parameters} we describe several specific parameter instantiations which lead to hardness results for (sparse) \klpn{} and \klwe{} based on popular assumptions for the hardness of standard \lpn{} and  \lwe{.
We end with our application to noisy tensor completion in \cref{sec:tensorcompletion}.



% \paragraph{LPN:}
% One of the most popular instances of random noisy linear equations over finite fields is the binary case of $q = 2.$ Under certain distributional assumptions (to be described shortly), no known algorithm takes time less than $\exp(\Omega(n/\log n)),$ suggesting extremely strong hardness. 
% % When $a_1, a_2, \ldots, a_m,s\iidsim\unif(\{0,1\}^n)$ and $e_1, e_2, \ldots, e_m\iidsim \Bernoulli(1/2 - \gamma),$ this problem is known as \emph{Standard Learning Parity of Noise} (Standard \lpn). The best known algorithm for this time takes time  \cite{BKW} and there is an $\exp(\Omega(n))$ lower bound in the SQ model \cite{kearns98sq}, suggesting a near-exponential hardness of the problem. 
% % The hardness of \lpn has proven extremely useful to theoreticians. 
% From the \lpn assumption, one can construct one-way functions, secret key identification schemes \cite{krzysztof12cryptoLPN}, bit commitment schemes \cite{abhishek12comitments} and many others (see \cite{krzysztof12cryptoLPN} for more applications to cryptography). In learning theory, \lpn takes a central role in understaidng the limitations of the statistical-query model \cite{kearns98sq,BKW}  and has found applications to lower-bound constructions for
% learning probabilistic finite automata with an evaluator \cite{kearns94learnability}, certain classes of graphical models \cite{mossel06phylogeny,bresler19bolzmann} and many others.

% \paragraph{LWE:}
% Another common instance is the case of Learning With Errors (LWE) when the modulus $q$ is ``large,'' typically at least polynomial in $n$ \cite{regev05LWE}. 
% % In Standard LWE,  $a_1, a_2, \ldots, a_m,s\iidsim\unif(\mathbb{Z}_q^n)$ and $e_1, e_2, \ldots, e_m$ are independently sampled from a discrete Gaussian distribution. 
% The learning with errors problem has revolutionized cryptography, with applications to fully homomorphic encryption \cite{brakerski11fhe}, non-interactive zero-knowledge proofs \cite{canetti19fiatshamir}, public-key encryption \cite{regev05LWE}, and succinct non-interactive argument systems \cite{jin24snarg} (see \cite{peikert16decade} for more applications to cryptography). More recently, the hardness of \lwe has been used to show hardness of various statistical problems such as learning Gaussian mixture models \cite{bruna21clwe,gupte2022continuous}, learning (intersections of) halfspaces \cite{klivans06cryptographic,tiegel23agnostic,tiegel24intersection}, learning periodic neurons \cite{zadik24neurons}, and others. What makes hardness of statistical problems based on \lwe prticularly appealing is that even though \lwe is an average-case problem, under certain distributional assumptions on $A, s, e,$ it inherits a worst-case hardness from standard lattice problems \cite{regev05LWE,peikert09publickey}.


==> FastTechOverview_new.tex <==
We next give an overview of the proof of our main theorem, namely \cref{thm:maininformal}.
% We first focus on the case when the distribution on the support is deterministically 1.
% We show how to achieve arbitrary distribution on the support as well as varying support sizes at the end of this section.

\subsection{The High-Level Approach: Linear Mapping from Dense to Sparse Equations}%Gadget Matrices}

In what follows, we denote the input to the dense problem by $(B,y)$ and the input to the sparse problem by $(A,y')$.
Suppose we are given $(B,y)$ such that $B$ is uniform over $\mathbb{Z}_q^{m \times L}$ and we want to solve one of the decision/search/refutation problems given access to an oracle for the same problem in the sparse setting.
The high-level idea is to transform each dense equation to a sparse one in a way that preserves the approximate linear relation $b_i ^\top s\approx y$ (or absence thereof) between ``coefficients'' $b_i$ in row $i$ of $B$ and the label $y_i$.

A common approach in the literature towards this end (e.g. \cite{boneh13bit} for binary LWE, and \cite{jain24sparseLWE} for sparse LWE in certain regimes, discussed in \cref{sec:priorreduction}) is to map the coefficient vector of each equation.
If we can find a linear mapping, this will preserve the linear relation between the coefficient vector and the label.
More specifically, we aim to find a matrix $G \in \mathbb{Z}_q^{n \times L}$ (we sometime refer to this as a \emph{gadget} or \emph{decoding matrix}) such that given a sample $(b_i, y_i) \in \mathbb{Z}_q^L \times \mathbb{Z}_q$, we can efficiently find a $k$-sparse $a_i\in \mathbb{Z}_q^{n}$ such that $a_i^\top G = b_i^\top$.
Note that given this, it holds that %when $y_i \approx b_i^\top s$ for some vector $s$, this implies that $y_i \approx a_i^\top (Gs)$, that is, the approximate linear relation is preserved.
%this equation implies
\begin{align}
\label{eq:gadgeteq1}
y_i \approx b_i^\top s \text{ for some } s 
% \text{ if and only if } 
\quad \Leftrightarrow \quad y_i \approx a_i^\top (Gs) \text{ for some } s. %b_i^\top s = (a_i^\top G)s = a_i^\top (Gs).
\end{align}
Further, it should hold that the sparse equation has the correct distribution, i.e., that $a_i$ is uniform over $k$-sparse vectors in $\mathbb{Z}_q^n$.
That is, we require the following property:
\begin{align}   
\label{eq:gadgeteq2}
    \text{If }b_i\sim\unif(\mathbb{Z}_q^L), \text{ then }a_i \text{ is a uniformly random }k\text{-sparse vector in }\mathbb{Z}_q^{n}.
\end{align}


We refer to the process of computing $a$ given $b$ as the \emph{decoding algorithm}. (Indeed, a watchful reader would already have seen the analogy with syndrome decoding in coding theory).
We claim that such a primitive can imply a reduction between all of the decision/search/refutation versions.
We illustrate this here for the search task, and refer to~\cref{sec:reduction_for_all_three_tasks} for the other two tasks.\footnote{Crucially, for the refutation task we need that \emph{almost all} of the equations are mapped successfully with high probability, while this is not necessary for decision and search. See~\cref{sec:reduction_for_all_three_tasks} for details.}
Assume that $y_i = b_i^\top s + e_i$ for some error term $e_i$.
Then, we can compute the mapped equation $y_i' = y_i + a_i^\top z$, where $z \in \mathbb{Z}_q^n$ is drawn uniformly at random.
It holds that
\[
    y_i' = y_i + a_i^\top z = b_i^\top s +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i \,,
\]
where we use the same $z$ for each sample. The only role of $z$ is that the final secret $Gs + z$ is uniform over $\Z_q^n$ and independent of everything else.
Thus, given a search oracle for the sparse version we can recover $Gs + z$ and hence also $Gs$.
If $G$ is full-rank we can then recover $s$. 
%\gb{Make clear that there is a single $z$ used for all equations and that the point is to make $Gs+z$ a uniformly random secret.}


%\stefanc{additional comments gadget matrices, in particular, it should become clear already that we want $L = \omega_n(k)$}
%\kirilc{ I think this sentence is unnencessary (and wrong):
%Our main contribution is to show that such an algorithmic primitive indeed exists.}
%\stefanc{Sounds good}

%Note that an appealing property of this approach is that it preserves the error distribution.



%The quality of the reduction will depend on how large $L$ is in comparison to $n$. 
%In particular, to obtain as tight a reduction as possible, we want $L$ to be large, ideally on the order of $k \log n$.
%Since (near-)exponential hardness of the dense problem then implies (near-)$n^k$ hardness for the sparse problem.



% up to lower order $\poly(\log k, \log\log n)$ factors. 
% \gb{This last sentence feels out of place unless it's connected to the prior sentence. Here's a suggestion for an alternative:}\kb{I agree. i further modified} In the rest of this section, we show that this upper bound can be nearly achieved.  (which is small in the regime that $q$ is at most polynomial in the initial dimension $L,$ in which case we obtain $\frac{k\log n}{\log q} = \frac{k\log n}{\}$). 

%\stefanc{One thing I find slightly confusing is that the entropy argument above treats $G$ as deterministic, is there a similar argument for random $G$?}
%\gb{we can make the following argument for random $G$. 1. consider all $m$ equations, 2. it's the same $G$ for all equations, and $G$ has entropy $ nL\log q$. This implies that $m L\log q\leq mk\log n + nL\log q$. So as long as $m\gg n$, essentially the same inequality holds. We could always add in a footnote saying that the randomness of $G$ makes no difference amortized over the samples.}\kb{ re: @Guy,  I am not sure I understand this comment. We never use a random $G.$ The randomness is only used to generate a $G.$ That is, if someone were to give me a deterministic ``good decoding matrix $G$' this would work just as well.}
%\gb{But you \emph{could} use a random $G$ if you wanted to, which might help make the resulting $a$ look more random to the black box. I'm just pointing out that there isn't enough randomness in $G$ to make a difference to the entropy argument.}
%\stefanc{Sounds good! I added a footnote.}

%\stefanc{This argument also shows that we only get an improvement over JLS24 if $q$ is much smaller than any polynomial in $n$. Should we state this more prominently somewhere? I think for the above argument it makes sense to add that for typical hardness assumptions $q = \poly(L)$, bc if people try to plug in $q = \poly(n)$, they might get confused. I don't really have a sense what kind of modulus you'd ideally want for the sparse variant}

%The key step in this approach is to design a gadget matrix $G\in \mathbb{Z}_q^{n\times L}$ for which the decoding step can be performed efficiently for as large $L$ as possible.

% We first describe how this enables reductions for all of decision, search, and refutation and then explain how to construct the gadget matrix and implement the decoding algorithm.





% Assuming this, the reduction works as follows:
% On input $\{(b_i,y_i)\}_{i=1}^m$, let $\{a_i\}_{i=1}^{m_1}$ be the successfully decoded $b_i$.
% If $m_1 < (1-o(1)) m$ output $\phi = 1$.
% Else, run the sparse refutation algorithm on $\{(a_i,y_i)\}_{i=1}^{m_1}$ (note that we do not change $y_i$).
% If it outputs $\phi'$ output $\phi = \phi' + o(1)$.
% Note that $\phi$ is always a correct upper bound: 1 is always an upper bound, and if $m_1 \geq (1-o(1))m$ at most a $(\phi' + o(1))$-fraction can be satisfiable.
% Else, there exists an $s$ such that $y_i = a_i^\top s$ for a larger than $\phi'$-fraction of the successfully decoded samples.
% Thus, the upper bound output by the sparse refutation algorithm cannot be correct.
% Note that with high probability $\phi$ will also be small, assuming that $\phi'$ is small with high probability (since we only output the naive upper bound 1 with probability $o(1)$).
% I.e., the strength of the refutation algorithm is preserved.

%Further, if $y_i$ was independent and uniform over $\mathbb{Z}_q$ to begin with, then so is $y_i + a_i^\top z$.
%If $y_i = b_i^\top s + e_i$, then $y_i + a_i^\top z = a_i^\top (Gs) +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i$ by \cref{eq:gadgeteq1} and $Gs + z$ is uniform over $\mathbb{Z}_q^n$.


\begin{comment}
\stefanc{The fact that the error is preserved should also imply that you can reduce between refutation problems, because the fraction of satisfied equations is preserved (up to the negligible fraction of samples you drop during the reduction)}

The high-level idea is to find some convenient gadget matrix $G\in \mathbb{Z}_q^{n\times L}$ and to solve $B = AG$ in such a way that $A$ has the correct  distribution. This is done sample by sample. That is, for each $b_i,$ one separately solves $a_i^\top G = b_i^\top.$ If one achieves this, one will be left with the following variables. $A, B = AG, y = Bs + e.$ Then, $y = AGs + e = As' + e$ where $s' = Gs$ is the new secret. A standard trick to make the new secret uniform is to draw a fresh $z\sim \unif(\mathbb{Z}_q^n)$ and add $Az$ to $y,$ thus $s_1 = s+ z\sim \unif(\mathbb{Z}_q^n).$
Hence, one obtains $(A, As_1 = e).$ The key step is to choose a gadget matrix $G$ such that one can solve $a^\top G = b^\top$ \emph{efficiently} in such a way that when $b\sim \unif(\mathbb{Z}_q^L),$ it is the case that $a$ is uniformly random $k$-sparse.
\end{comment}


\subsection{Prior Gadget Matrix Constructions and Challenges}
\label{sec:priorreduction}
The only prior work that we are aware of which reduces standard (dense) noisy linear equations to sparse ones is 
\cite{jain24sparseLWE} in the case of  \lwespace (and large-field LPN).
The authors follow the gadget matrix approach outlined above with $L = k$ and $G \in \mathbb{Z}_q^{n \times k}$ the Vandermonde matrix, i.e., whose $i$-th row is equal to $(i^0, i^1, i^2, \ldots, i^{k-1})$.

To solve $a^\top G = b^\top$ on input $b\sim\unif(\mathbb{Z}_q^k)$ such that $a$ is a uniformly random $k$-sparse vector, 
they first draw a uniformly random support $S\in \binom{[n]}{k}$ \emph{independently} of $b$.
Then, they restrict $a$ and $G$ to coordinates $S$ and solve the equation $a^{\top}_SG_{S\times [k]} = b^\top$.
Whenever $q\ge n,$ \emph{every $k\times k$ minor of $G$ is of full rank} and, hence, a unique solution for $a_S$ exists.
Since $b$ is uniform over $\mathbb{Z}_q^k$, it is easy to check that $a_S$ is also uniform over $\mathbb{Z}_q^k$, so $a$ has the correct distribution.
Overall, the reduction of \cite{jain24sparseLWE} shows that $n$-dimensional $k$-sparse \lwe{} is at least as hard as $k$-dimensional \lwe; assuming exponential hardness of \lwespace implies that the $k$-sparse version takes time at least $2^{\Omega(k)}$.

We outline two ways in which one might hope to improve over this reduction:

\paragraph{Desideratum 1: Small Values of $k.$}
% As discussed before, even assuming exponential hardness of \lwe, 
As noted just above, the hardness implied by \cite{jain24sparseLWE} for $n$-dimensional \klwe{} is at best only $2^{\Omega(k)}$, which does not yield any hardness against polynomial-time (in $n$) attacks when $k = O(\log n)$. %This is a concern because certain protocols such as the linear homomorphic encryption based on sparse \lwe{} has overhead  $O(k\log \log q)$ and rate $O(k)$ and, thus, improves on previous work only in the regime $k = (\log n)^{o(1)}$ \cite{jain24sparseLWE}. The $2^{\Omega(k)}$ hardness also falls short of the conjectured $n^{\Omega(k)}$ lower bound that is frequently assumed and known to be true in restricted models of computations such as the SoS hierarchy~\cite{grigoriev2001linear,schoenebeck2008linear} and the SQ model for the related sparse \lpn problem (and, as we show, in the low-degree framework \cref{lemma:lowdegreeinzq} for sparse \lwe). 
%\gb{This paragraph is redundant and belongs in "unsatisfactory state of affairs". The only needed sentences are the first two, JLS gives $2^k$ and we need $n^k$.}
%\stefanc{I commented out the rest}
%\stefanc{I tried making the argument below a bit more concise and phrasing it in a way that ties it back in to the entropy argument we made above, here's the new version:}
It is instructive to analyze where their reduction is loose.
As an intermediate step of transforming a dense $b \in \mathbb{Z}_q^L$ to a $k$-sparse $a \in \mathbb{Z}_q^n$, they compute a dense vector $\tilde{a} \in \mathbb{Z}_q^k$ such that $\tilde{a}^\top \tilde{G} = b$, for some deterministic matrix $\tilde{G}$.
Note that the entropy of $b$ is equal to $L \log q$ and this must be smaller than the entropy of $\tilde{a}$.
Since the entropy of $\tilde{a}$ is at most $k\log q$, we must have $k \log q \geq L \log q$ and hence $L \leq k$. This approach leaves the entropy of the support location of $a\in \mathbb{Z}_q^n$ unexploited. There are $\binom{n}{k}$ choices for the support of $a,$ which yields $\log \binom{n}{k}\approx k\log n$ additional bits of entropy. Thus, if one simply requires $a^\top G = b^\top$ (instead of $\tilde{a}^\top \tilde{G} = b$), the corresponding entropy calculation is $k \log n + k\log q\ge L\log q,$ allowing for larger values of $L.$
We record this as a guiding principle:
\begin{equation}
\label{eq:P1}
\tag{P1}
\textit{
        For small $k,$ when solving $a^\top G = b^\top$, one must choose the support of $a$ based on $b$. 
    }
\end{equation}

Note that a similar entropy does give \emph{some} limitations for general decoding matrices when $L = \omega(k).$
Since the entropy of $a$ is at most $k \log n$ it must hold that $L \log q \leq k \log n$, i.e., $L \leq k \log n / \log q$.\footnote{In this argument we implicitly assumed that $G$ is deterministic. Since we use the same $G$ for all equations, even for a random $G$ the average entropy added on any single equation is at most $\tfrac{n L \log q}{m}$ which is negligible for all parameter settings we consider.}
We will show that this upper bound can nearly be achieved.
In particular, we will be able to choose $L = k\log n/\poly(\log k,\log\log n, \log q)$.


This task can be interpreted as a sampling version of 
the popular $k$-SUM problem, in which given $n$ vectors  in $\mathbb{Z}_q^L$ and a target $b$ one needs to find $k$ of them that sum to $b.$
This problem is believed to take time at least $\min(n^k, 2^{L/\log k})$ \stefanc{Is this stated correctly? I just rephrased what was there previously} in both average-case and worst-case settings ~\cite{brakerski2020hardness,patrascu10fastersat,abboud22sethksum} under worst-case lattice problems or the exponential time hypothesis.
Since we are searching for a $\poly(n)$-time algorithm, this poses a serious obstacle.
In particular, since we furthermore want to \emph{sample} from the $k$-SUM solutions. 
We circumvent this hardness by exhibiting a gadget matrix $G$ that allows for efficient sampling.\kirilc{I am a little confused how this paragraph ended up here}

% Stefan: previous version
\begin{comment}
\stefanc{Previous version:}
So, is there some inefficiency in the reduction of \cite{jain24sparseLWE}?
The inefficiency comes from the fact that the support $S$ 
% is not exploited because  
is drawn independently from $b$. As a simple illustration, even if one deterministically draws $S = \{1,2,\ldots, k\}$ at each step, the reduction of \cite{jain24sparseLWE} still goes through (and this makes sense since one will just obtain an instance of $k$-dimensional \lwe{} in this way). 
However, if one wants a quantitative improvement and reduce standard $L$-dimensional \lwe{} to $n$-dimensional $k$-sparse \lwe{} for some $L = \omega(k),$ the \emph{entropy of the support needs to be used}.
Indeed, note that the number of vectors $b$ over $\mathbb{Z}^L_q$ is $q^L.$
The number of $n$-dimensional $k$-sparse vectors $a$ is $\binom{n}{k}q^k$ where the $\binom{n}{k}$ contribution is from the support location and $q^k$ from the entries on the support.
If $a^\top G = b^\top$ has a solution in $a$ for any $b,$ it must be the case that $\binom{n}{k}q^k\ge q^L$ or equivalently $\binom{n}{k} \ge q^{L-k} = q^{L(1-o(1))}.$
This shows that the bulk of the entropy should come from the $\binom{n}{k}$ factor corresponding to the support location. 
\gb{this seems to only be true if $n\gg q$, no?}
\stefanc{Yes, I think this is related to my comment about $\log q$ in the previous paragraph.}
One cannot afford to lose this entropy by drawing the support independently from $b.$
We record this principle:
\begin{equation}
\label{eq:P1}
\tag{P1}
\textit{
        For small $k,$ when solving $a^\top G = b^\top$, one must choose the support of $a$ based on $b$. 
    }
\end{equation}
\end{comment}

\paragraph{Desideratum 2: Small Moduli.}
We would like our reduction to work also for small moduli, and in particular for $q = 2$ as in the case of \lpn.
Note that a key step in the reduction of \cite{jain24sparseLWE} is the inversion of an arbitrary $k \times k$ sub-matrix of $G$, which requires every $k\times k$ minor of $G$ to be full rank.
Such matrices are known as \emph{maximum distance separable} and in the regime $n\ge k,$
conjecturally, cannot exist if $q< n-2$ (e.g. \cite{huffman03fundamentals}). Hence, one cannot hope for a reduction in the important case of \lpn{} using the approach of \cite{jain24sparseLWE}.
Our approach will also rely on inverting (smaller-sized) linear systems, yet we will carefully brute-force over appropriate sub-instances and thus do not need the corresponding matrix to be full-rank.

% \paragraph{Challenge 3: Other Distributions on the Support.} Finally, it is unclear how to 
We would also like to be more versatile, e.g. obtain sparse vectors $a_i$ with distribution on the support different from uniform over $\mathbb{Z}_q^k$. As one example, our application to the hardness of tensor completion from \lwespace{} requires \emph{binary} $k$-sparse coefficients $a_i$. This does not seem possible using the approach in \cite{jain24sparseLWE}.
% , in the current work, for example, we need binary $k$-sparse samples $a_i$ for the application to tensor completion.

\subsection{A Toy Reduction for Block-wise Sparsity}

A gadget mapping dense $L$-dimensional vectors to {\em blockwise} $k$-sparse $n$-dimensional vectors is not hard to construct. A blockwise sparse vector is one whose coordinates are divided into $k$ blocks, each of which has a single non-zero coordinate. Indeed, for a parameter $t=L/k$, let $H \in \mathbb{Z}_q^{t \times q^{t}}$ denote a matrix whose columns are all the vectors in $\mathbb{Z}_q^{t}$. Then, we will let the decoding gadget $G = I_k \otimes H \in \mathbb{Z}_q^{t k \times q^{t}k}$. First of all, since $L=t k$ and $n= q^{t} k$, notice that $$ L = \frac{k\log (n/k)}{\log q} \,.$$
Secondly, given an $L$-dimensional vector $b$, one can decode each block of $t$ coordinates of $b$ into a unit vector in $q^{t}$ dimensions. Concatenating the unit vectors gives us a block-wise sparse $n$-dimensional vector $a$ such that $a^\top G = b^\top$. 
%While block-wise sparsity may suffice for some applications, we are not content with it. 

Permuting the coordinates might seem to suffice to turn blockwise sparsity into true sparsity. However, since the same permutation has to be used for all $m$ samples, the blockwise structure starts becoming apparent once one sees sufficiently many samples. For example, given $\omega(n^2)$ samples, every two coordinates $i,j$ appear in some row of the public matrix $A$ when the supports are uniformly random $k$-tuples. This property is not shared by the blockwise model for any number of samples under any permutation.

To decode to random sparse vectors, we need a cleverer idea which we describe next.



\subsection{Overview of Our Reduction to Sparse Equations} 
\label{sec:nontechnicaloverview}
We begin by explaining the reduction in the case that the distribution on the support is deterministically equal to 1, which captures both \klpn{} and \emph{binary} \klwe.
At the end of this section, we explain how a simple modification addresses arbitrary distributions on the support.


\paragraph{Motivation for Our Reduction: Translation of Natural Languages.}

A key step in our reduction will be to split the decoding problem into smaller sub-problems and then combining the solutions to these sub-problems into a solution to the full problem.
Our approach will be reminiscent of how translation of natural languages works:
The full problem can be thought of as translating a sentence (from the ``dense'' to the ``sparse'' language) and the sub-problems as translating a word (which will be done using a dictionary).
We use the grammar of the respective languages to (a) determine the sub-problems and (b) combine their solutions.
Intuitively, translating word by word should be easier than translating a whole sentence at once since it has much lower complexity.

A word in the ``dense'' language is just a substring and the grammar is given by concatenation.
It will be more convenient to think of a word in the $k$-``sparse'' language as just a collection of $k$ indices over some small domain.
A sentence in this language is a $k$-tuple over a much larger domain.
Our key contribution is a grammar for the ``sparse'' language:
That is, we show how to combine multiple $k$-tuples over a small domain to a single $k$-tuple over a much larger domain.
A key property is that the sparsity remains the same, e.g., simply concatenating them would result in too large a blow-up of the sparsity for our applications.



\paragraph{Representing Uniformly Sparse Solutions as Steps of Random Walks.}

Consider for a moment the reverse direction of what we are trying to show.
I.e., given a uniformly random $k$-sparse vector $a$ in dimension $n$, design a matrix $G$, such that $a^\top G = b \in \mathbb{Z}_q^L$ and the distribution of $b$ is (close to) the uniform distribution over dense vectors.
Note that, thinking of the entries of $a$ as a $k$-tuple with repetitions allowed, this has a natural interpretation as the following random process:
Start with the all-zeroes vector and for $k$ steps, choose a row of $G$ at random and add it to the current state.
In particular, we can think of the steps of this random walk, i.e., the entries of the $k$-tuple, as an implicit representation of $b$ (together with the gadget matrix $G$).
The task of finding a good gadget matrix $G$ is now a task of designing update rules of a random walk such that the walk mixes quickly.

Taking this viewpoint, it becomes clear that \emph{redundancy} (in terms of the number of steps we take) is key to achieve uniformity of the final state/vector.
In particular, the most canonical random walk over $\mathbb{Z}_q^L$ is as follows: at every step, choose a random coordinate and add a uniformly random element over $\mathbb{Z}_q$ to it.
As we will see, this also has a very natural encoding as a gadget matrix $G$.
This walk converges to an almost uniform state in roughly $L (\log L + \log q)$ steps.
Conversely, we could hope that the reverse direction is also true, i.e., given a uniform vector $b$, its implicit representation in terms of steps of this walk is close to uniform over all $k$-tuples, as long as $k \approx L (\log L + \log q)$.
We could then try to decode this $k$-tuple into a $k$-sparse vector.

Even assuming uniformity of this implicit representation, and additionally that we can efficiently find one, this has the obvious drawback that the size of the representation is even larger than the initial dimension.
And thus, we will likely not be able to decode it into a sparse vector (where the sparsity is supposed to be much smaller than the dimension).
However, one of our main insights is that that this line of reasoning still applies to sub-strings of the input $b$.\footnote{The idea to split the problem into smaller sub-problems is similar to the celebrated BKW algorithm \cite{BKW}.}
In particular, writing $b = (b_1, \ldots, b_t)$, our reduction rests on the following two properties:
\begin{enumerate}
    \item Given a uniform $b_i \in \Z_q^{h}$, we can efficiently compute an implicit representation of $b_i$ that is (close to) uniform over all $k$-tuples (over some small domain) such that $k \approx h (\log h + \log q) \ll n$.
    \item We can efficiently combine all implicit representations of the $b_i$ to a representation of $b$ as a $k$-tuple over $[n]$.
    Further, if all initial representations are uniform, the final one will be as well.
\end{enumerate}
Crucially, the size of the representation does not increase in the last step (only the size of the domain).
We can easily decode the final $k$-tuple into a $k$-sparse vector.


\paragraph{Word Decoding: Finding Uniform Implicit Representations of Small Sub-Problems.}

More formally, we represent each $b\in \mathbb{Z}_q^L$ as $(b_{1}, b_{2}, \ldots, b_{t})$, where each $b_i \in \mathbb{Z}_q^h$.
% We will think of each $b_i$ as a concatenation of $t$ independent strings  of length $h.$ 
We will decode each $b_{j}$ into a $k$-tuple of indices over $[hq]^k$ via a smaller gadget matrix $V \in \mathbb{Z}_q^{hq \times h}$ (this is the dictionary mentioned above).
The following gadget matrix corresponds to the lazy random walk over $\mathbb{Z}_q^h$.
%As we will need to solve $k$-SUM over this $V,$ it is natural that we want $V$ to have a very simple explicit structure. We take $V$ to contain all multiples of the identity:
\begin{align*}
    V= 
    \begin{pmatrix}
      0 \times I_h\\
      1\times I_h\\
      \quad \vdots\\
      (q-1)\times I_h
    \end{pmatrix}.
\end{align*}
We call the $hq$ rows $V_{1,:}, V_{2,:},\ldots, V_{hq,:} \in \mathbb{Z}^h_q$ words.
%Here, $h$ is the word length.
We want to find $\xi_j = (\xi_j(1),  \ldots, \xi_j(k)) \in [hq]^k$ such that the sum of the rows of $V$ indexed by $\xi_j$ is equal to $b_j$ %$$\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}\,.$$ % (hereon, we identify $k$-sparse binary vectors with $k$-tuples of indices). 
Furthermore, if $b_j$ is uniform over $\mathbb{Z}_q^h$, we will require the marginal distribution of $\xi_j$ to be uniform over $[hq]^k$.
In particular, consider the set of all such $\xi_j$
\begin{equation}
\label{eq:preimagedef}
\begin{split}
\Preimage_{V}(b) \coloneqq \Set{(\xi(1), \xi(2), \ldots,\xi(k))\in [hq]^k\suchthat \sum_{\psi = 1}^k V_{\xi(\psi).:} = b}.
\end{split}
\end{equation}
We will show that (i), we can efficiently sample a uniform element from $\Preimage_{V}(b)$ and (ii), for a uniformly random $b$, this is close to uniform over all $k$-tuples over $[hq]$.
We can make the distribution exactly uniform by a simple rejection sampling step.

Towards (i) we show the following lemma.
\begin{lemma}[Efficient preimage sampling]
\label{lem:samplingintro}
% There exists an algorithm (\cref{alg:samplingfrompreimage}) with the following property.
On input $k>h+2$ and $b \in \mathbb{Z}_q^h,$ there exists an algorithm (cf.~\cref{alg:samplingfrompreimage}) that outputs a uniformly random element of $\Preimage_V(b).$ The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}
On a high level, this can (roughly) be achieved by sampling indices uniformly at random (from $[hq]$) until the number of indices left matches the number of coordinates that differ between the current state, i.e., the sum of rows of $V$ indexed by the current indices, and $b$.
The choice of the remaining coordinates is then fixed.
Permuting them randomly will result in a uniformly random element from the preimage.

%When combining the different words into sentences, a key property will be that $\xi_j(1),  \ldots, \xi_j(k)$ are (nearly) independent and uniform over $[hq].$ To guarantee this, a key property will be that each $\Preimage_V(b)$ is of nearly equal size. Otherwise, $k$-tuples $\xi_j(1),  \ldots, \xi_j(k)$ corresponding to $b$ with large (respectively, small)
%$\Preimage_V(b)$ will be under-represented (respectively, over-represented). Again, the simple structure of $V$ can be utilized to show the following fact.
Note that the sets $\Preimage_{V}(b)$ partition the set of all $k$-tuples over $[hq]^k$.
Thus, if all of these parts have (roughly) the same size, outputting a random element from one of them will be close to uniformly random (on input a uniformly random $b$).
More specifically, we show the following.
\begin{lemma}[Uniformity of preimage size]
\label{lem:nearuniformityintro}
    Suppose that $k \ge 4h(\log h +\log q +  \log (1/\psi))$ where $\psi\in (0,1)$ is any real number. Then, for each $u \in \mathbb{Z}_q^h$,
    $$
    \frac{(1-\psi)(hq)^k}{q^h}\le 
    |\Preimage_V(u)|
    \le 
    \frac{(1+\psi)(hq)^k}{q^h}.
    $$
\end{lemma}
We give the proof in \cref{sec:randomwalkproof}, which follows by analyzing the point-wise convergence of the lazy random walk on $\mathbb{Z}_q^h$. Note that it is well-known that this walk converges to the uniform distribution in total variation distance after roughly $h (\log h + \log q)$ steps. For our applications, the stronger, point-wise converges guarantee is crucial.
In particular, trying to deduce a point-wise converge bound from the total variation bound would require $k \gtrsim h^2$ which would result in a much looser lower bound.
% 
For reasons that will become clear, we will choose $\psi = o(1/t),$ say $\psi = (ht)^{-2}.$

In order to make the output tuples exactly uniform, we will use a simple rejection-based method that rejects each $b_j$ with probability $$1 - \frac{|\Preimage_V(b_j)|}{{(1+\psi)(hq)^k}/{q^h}},$$ which is a well-defined probability and is at most 
$2\psi$ under the guarantee of \cref{lem:nearuniformityintro}.
To make this algorithmically efficient, we need to be able to compute $|\Preimage_V(b_j)|.$
This will follow by first observing that by symmetry considerations, the size of the set only depends on the number of non-zero entries of $b_j$.
Then, the size can be efficiently computed via dynamic programming.
\begin{lemma}[Computing preimage size]
\label{lem:sizeestimationintro}
There exists an algorithm (cf.~\cref{alg:sizeestimation}) that on input $k$ and $b \in \mathbb{Z}_q^h,$ outputs
$|\Preimage_V(b)|.$
The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}

% Stefan: Previous Version
\begin{comment}
\paragraph{Word Decoding: Splitting into Small Sub-Problems That Can Be Solved Efficiently.}
We will decompose the problem into $t$ sub-problems by splitting the string $b$ into $t$ equal parts (similar to the celebrated BKW algorithm \cite{BKW}).
These parts of size $h\coloneqq L/t$ will be small enough that we can efficiently find a representation using $k$-tuples in each part, and these will then be carefully combined.
%Then, we will combine these $t$ small sub-problems.
It will be convenient to work with $k$-tuples of indices for now, i.e., allow repeated indices. We will be able to show that only a negligible fraction actually has repeated indices, so that we can represent most of them as $k$-sparse vectors.
% \stefanc{I would mention that again we need sth like $r^k \geq 2^(L/t)$ -> need $t$ not too small}

More formally, represent each $b\in \mathbb{Z}_q^L$ as a concatenation of $t$ uniform independent strings $b = (b_{1}, b_{2}, \ldots, b_{t})$ in $\mathbb{Z}_q^h$.
% We will think of each $b_i$ as a concatenation of $t$ independent strings  of length $h.$ 
We will decode each $b_{j}$ into a $k$-tuple of indices over $[hq]^k$ via a smaller gadget matrix $V \in \mathbb{Z}_q^{hq \times h}$ (this is the dictionary mentioned above). As we will need to solve $k$-SUM over this $V,$ it is natural that we want $V$ to have a very simple explicit structure. We take $V$ to contain all multiples of the identity:
\begin{align*}
    V= 
    \begin{pmatrix}
      0 \times I_h\\
      1\times I_h\\
      \quad \vdots\\
      (q-1)\times I_h
    \end{pmatrix}.
\end{align*}
We call the $hq$ rows $V_{1,:}, V_{2,:},\ldots, V_{hq,:} \in \mathbb{Z}^h_q$ words.
%Here, $h$ is the word length.
We want to find $\xi_j = (\xi_j(1),  \ldots, \xi_j(k)) \in [hq]^k$ such that $$\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}\,.$$ % (hereon, we identify $k$-sparse binary vectors with $k$-tuples of indices). 
Furthermore, if $b_j$ is uniform over $\mathbb{Z}_q^h$, we will require the marginal distribution of $\xi_j$ to be uniform over $[hq]^k$.
We achieve this by outputting a uniformly random $\xi_j$ that satisfies $\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}$.

Here, we take the opportunity to introduce some useful notation:
\begin{equation}
\label{eq:preimagedef}
\begin{split}
\Preimage_{V}(b) \coloneqq \Set{(\xi(1), \xi(2), \ldots,\xi(k))\in [hq]^k\suchthat \sum_{\psi = 1}^k V_{\xi(\psi).:} = b}.
\end{split}
\end{equation}
The simple structure of $V$ allows for extremely efficient sampling from the preimage of $b.$

\begin{lemma}[Efficient preimage sampling]
\label{lem:samplingintro}
% There exists an algorithm (\cref{alg:samplingfrompreimage}) with the following property.
On input $k>h+2$ and $b \in \mathbb{Z}_q^h,$ \cref{alg:samplingfrompreimage} outputs a uniformly random sample from $\Preimage_V(b).$ The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}

When combining the different words into sentences, a key property will be that $\xi_j(1),  \ldots, \xi_j(k)$ are (nearly) independent and uniform over $[hq].$ To guarantee this, a key property will be that each $\Preimage_V(b)$ is of nearly equal size. Otherwise, $k$-tuples $\xi_j(1),  \ldots, \xi_j(k)$ corresponding to $b$ with large (respectively, small)
$\Preimage_V(b)$ will be under-represented (respectively, over-represented). Again, the simple structure of $V$ can be utilized to show the following fact.

\begin{lemma}[Uniformity of preimage size]
\label{lem:nearuniformityintro}
    Suppose that $k \ge 4h(\log h +\log q +  \log (1/\psi))$ where $\psi\in (0,1)$ is any real number. Then, for each $u \in \mathbb{Z}_q^h$,
    $$
    \frac{(1-\psi)(hq)^k}{q^h}\le 
    |\Preimage_V(u)|
    \le 
    \frac{(1+\psi)(hq)^k}{q^h}.
    $$
\end{lemma}
We give the proof in \cref{sec:randomwalkproof}, which follows by analyzing the point-wise convergence to the uniform distribution of a naturally occurring Markov chain over $\mathbb{Z}_q^h$.
% 
For reasons that will become clear, we will choose $\psi = o(1/t),$ say $\psi = (ht)^{-2}.$

In order to make the output tuples exactly equal, we will use a simple rejection-based method that rejects each $b_j$ with probability $$1 - \frac{|\Preimage_V(b_j)|}{{(1+\psi)(hq)^k}/{q^h}},$$ which is a well-defined probability and is at most 
$2\psi$ under the guarantee of \cref{lem:nearuniformityintro}.
To make this algorithmically efficient, we need to be able to compute $|\Preimage_V(b_j)|.$ Again, the simple structure of $V$ allows such a primitive:

\begin{lemma}[Computing preimage size]
\label{lem:sizeestimationintro}
There exists an algorithm, \cref{alg:sizeestimation}, which on input $k$ and $b \in \mathbb{Z}_q^h,$ outputs
$|\Preimage_V(b)|.$
The algorithm runs in time $\poly(k,h,\log q).$
\end{lemma}
\end{comment}

\paragraph{Sentence Decoding: Combining the Solutions of Small Sub-Problems.}
 We will think of concatenations of words as sentences.
 Each sentence will have exactly $t$ words.
 The rows of our final gadget matrix will be all possible sentences, of which there are $ (hq)^t$.

Let $n = (hq)^t$.
We will use the decodings $\{\xi_j\}_{j=1}^t$ of $\{b_{j}\}_{j = 1}^t$ obtained via the matrix $V$ to produce a $k$-tuple $\xi \in [n]^k = ([hq]^t)^k$ decoding of $b.$ The key insight is that $\{b_{j}\}_{j = 1}^t$ are $t$ iid vectors in $\Z_q^h$ and, hence, $\{\xi_j\}_{j=1}^t$ are $t$ iid tuples in $[hq]^k.$ In particular, $(\xi_j(\psi))_{1\le j \le t, 1\le \psi\le k}$ are $kt$ independent uniform integers in $[hq].$

By definition, $\xi$ should be uniformly random. We define $\xi(\psi)\coloneqq (\xi_1(\psi),\xi_2(\psi),\ldots, \xi_t(\psi))$ for $1 \leq \psi \leq k$ and $\xi= (\xi(1), \xi(2), \ldots, \xi(k)).$ Visually, we represent $\xi$ as the following matrix in $[hq]^{t\times k}.$
$$\xi = 
\begin{pmatrix}
    \xi_1(1) \; \xi_1(2)\; \ldots \; \xi_1(k)\\
    \xi_2(1) \; \xi_2(2) \; \ldots\; \xi_2(k)\\
    \vdots\\
    \xi_t(1)\; \xi_t(2)\; \ldots  \; \xi_t(k)\\
\end{pmatrix}.
$$
In it, each row corresponds to a decoded word (that is, $\xi_j(1), \xi_j(2), \ldots, \xi_j(k)$ is the $k$-tuple corresponding to $b_j$). Each column $\xi(\psi) = (\xi_1(\psi), \xi_2(\psi), \ldots, \xi_t(\psi))^\top$ corresponds to a $t$-tuple in $[hq]^t$ and, hence, can be treated as an index in $[(hq)^t] = [n].$ This is the $k$-sparse grammar we referred to.
Crucially, each of the $k$ indices (columns) are independent and uniform. Thus, we have managed to translate $b\in \Z_q^{ht}$ into $k$ uniform independent indices in $[(hq)^t] = [n],$ as desired. 

To finish, we put this in the language of gadget matrices and demonstrate a linear relationship between $b$ and $\xi.$ Let $G\in \mathbb{Z}_q^{n \times L}$ be such that its rows are indexed by $ (\phi_1, \ldots, \phi_t) \in [hq]^t$ and each row is defined by
\begin{equation}
\label{eq:gdefintro}
G_{(\phi_1, \phi_2,\ldots, \phi_t),:} = 
(V_{\phi_1,:},V_{\phi_2,:},\ldots, V_{\phi_t,:})\in \mathbb{Z}_q^{ht} = \mathbb{Z}_q^{L} \,.
\end{equation} 
In other words, $G$ contains all possible concatenations of $t$ words from $V.$
%We think of each $t$-tuple of words from $W$ as a sentence and, hence, $G$ consists of all possible sentences using $t$ words.
% We offer the following illustration for $t = 3$, where $\mathbbm{1}_r$ is the all-ones vector in $\mathbb{R}^r$
% \[\arraycolsep=8pt
% G(W) = \left(\begin{array}{ccc}
% w_1^\top \otimes \mathbbm{1}_r & w_1^\top \otimes \mathbbm{1}_r & W \\
% \vdots & \vdots & \vdots \\
% w_1^\top \otimes \mathbbm{1}_r & w_r^\top \otimes \mathbbm{1}_r & W \\
% \\
% \hline 
% \\
% \vdots & \vdots & \vdots \\
% \\
% \hline \\
% w_r^\top \otimes \mathbbm{1}_r & w_1^\top \otimes \mathbbm{1}_r & W \\
% \vdots & \vdots & \vdots \\
% w_r^\top \otimes \mathbbm{1}_r & w_r^\top \otimes \mathbbm{1}_r & W \\
% \end{array} \right)\,.
% \]



Since $\sum_{\psi = 1}^k V_{\xi_j(\psi),:} = b_{j}^\top$ holds for each $j$, it must be the case that 
\begin{equation}
\begin{split}
\label{eq:introsumingadget}
\sum_{\psi = 1}^k G_{\xi(\psi)} = \sum_{\psi = 1}^k
 \Big( V_{\xi_1(\psi),:},V_{\xi_2(\psi),:},\ldots, V_{\xi_t(\psi),:}\Big) &= \Big( \sum_{\psi = 1}^k V_{\xi_1(\psi),:},  \sum_{\psi = 1}^k V_{\xi_2(\psi),:},\ldots,  \sum_{\psi = 1}^k V_{\xi_t(\psi),:}\Big) \\
 &= \big( b_1^\top, b_2^\top, \ldots, b_t^\top\big) = b^\top\,.
 \end{split}
\end{equation}
Under a mild condition $k = o(\sqrt{n}),$ the birthday paradox shows that with high probability, all of the $\xi(\psi)$ are distinct. When this event holds we can represent $\xi$ as a (binary) $k$-sparse vector $a$ that is uniformly random (the non-zero coordinates of $a$ are indexed by $\xi(1), \xi(2), \ldots, \xi(k)$).
\eqref{eq:introsumingadget} is equivalent to $a^\top G = b^\top$ as desired.

%Ignoring the fact that there might exist $\psi_1\neq \psi_2$ such that $\xi(\psi_1) = \xi(\psi_2),$ we are left with uniform $k$-tuples over $G.$ Hence if $a \in \mathbb{Z}_q^n = \mathbb{Z}_q^{r^t}$ is such that $a(\xi(\psi)) = 1$ for all $\psi \in \{1,2,\ldots, k\}$ and $a(\zeta) = 0$ otherwise, we are left with a $k$-sparse vector $a$ such that $a^\top G = b^\top.$

% Stefan: Most of this is in the paragraph in the beginning, so we could remove this
\begin{comment}
\paragraph{Endgame.}
Altogether, we have $AG(W) = B$ and the matrix $A$ is drawn uniformly from the binary $k$-sparse  \lwe. Hence, we transform $(B, Bs + e)$ into $(A, AG(W)s + e).$ We are not done yet as the secret $Gs$ is not uniform over $\mathbb{Z}_q^{n}$ as it is in the column span of $G \in \mathbb{Z}_q^{n\times L}$ which is clearly not full rank ($L\ll n$). Nevertheless, we can simply choose a fresh $z\sim \mathbb{Z}_q^n$ and find $(A, A(Gs+z) + e).$  Now, $s_1 = Gs + z\sim \unif(\mathbb{Z}_q^n).$ 
 
This concludes the reduction for the decision problem in the case $\mathcal{D}\equiv 1^k.$ When reducing between the search and refutation problems, some extra steps are needed but these are mostly technical details. In particular, for search we require that $G$ is of rank $L$ and for refutation that even for worst case $b_j,$ the $k$-tuple $\xi_j(1), \xi_j(2), \ldots, \xi_j(k)$ consists of pairwise different indices with high probability.
\end{comment}

\paragraph{Other Distributions on the Support.} 
Given a vector $b\in \mathbb{Z}_q^L,$ we first solve the binary problem. That is, find a $k$-tuple $(i_1, \ldots, i_k) \in [n]^k$ such that the corresponding rows of $G$ sum to $b$.
If $b$ is uniform, then so is $(i_1, \ldots, i_k),$ as already mentioned.
%For each sample $b,$ we use the sentence-decoding matrix $G(V)$ to find some $k$-sparse binary $a$ such that $a^\top G(V) = b^\top$ whose support is furthermore uniformly distributed. Let the support be $(i_1, i_2, \ldots, i_k)\in [n]^k.$
Next, sample $\rho = (\rho_1, \rho_2, \ldots, \rho_k)\in (\mathbb{Z}_q\backslash\{0\})^k$ from $\mathcal{D}$.
Suppose that the row of $G$ indexed by $i_j$ corresponds to
\[
(\kappa_1(j)e^\top_{\Delta_1(j)},\kappa_2(j)e^\top_{\Delta_2(j)},\ldots, \kappa_t(j)e^\top_{\Delta_t(j)}) \,,
\]
where $\kappa_i(j) \in 
\mathbb{Z}_q$ and $\Delta_i(j) \in [h].$
We use the convention that the first $h$ (zero) rows of $V$ are $0e_1^\top,0e_2^\top,\ldots,0e_s^\top.$
Now, replace this index with the index $i_j'$ corresponding to
\[
(\kappa_1(j)\rho_j^{-1}e^\top_{\Delta_1(j)},\kappa_2(j)\rho_j^{-1}e^\top_{\Delta_2(j)},\ldots, \kappa_t(j)\rho_j^{-1}e^\top_{\Delta_t(j)})\,.
\]
Since $\rho_j \neq 0$, $i_j'$ is still uniform over $[n]$.
Suppose again that all $i_j'$ are distinct, we can show that this happens with high probability.
Let $a'$ be the vector with support $(i'_1, i'_2, \ldots, i'_k)$ such that $a'_{i'_j} = \rho_j$.
Then, $(a')^\top G = a^\top G = b^\top$ and clearly the support of $a'$ is uniform and the distribution on the support equal to $\cD$.

\paragraph{Variable Support Sizes.} Finally, we can also accommodate for varying support sizes. The reason is that all of our primitives - \cref{lem:samplingintro,lem:sizeestimationintro,lem:nearuniformityintro} only rely on $k$ being sufficiently large and, thus, it is enough to accommodate for the effectively smallest possible support size $k.$

More concretely,
suppose that the distribution of support sizes is $\mathcal{K}$ where with probability $1 - \eta$ with $\eta = o(1/m)$ the support size is at least $k_\minsf.$ Then, for each sample $b_i,$ we first draw $k_i\sim \mathcal{K}$ and then use the word-decoding and sentence-decoding procedures for $k_i.$
We can show that the $k$-tuples are still uniform for all $k_i \ge k_\minsf$ if the input $b$ is random.
With high probability, we never see $k_i< k_\minsf.$ More detail is given in \cref{sec:variablesupportsizes}.


\paragraph{Summary of Parameters.} We summarize the parameters for convenience of the reader.

\begin{equation}
\label{eq:parameters}
\begin{split}
& \textsf{PROBLEM PARAMETERS:}\\
& \quad\quad\quad k \text{ sparsity},\\
& \quad\quad\quad n \text{ target dimension},\\
& \quad\quad\quad L \text{ initial dimension},\\
& \quad\quad\quad q \text{ modulus}.\\
& \textsf{AUXILIARY PARAMETERS FOR REDUCTION:}\\
& \quad\quad\quad hq \text{ number of words in } V,\\
& \quad\quad\quad h \text{ word length in } V,\\
& \quad\quad\quad t \text{ sentence length}.\\
& \textsf{RELATIONSHIPS:}\\
& \quad\quad\quad n = (hq)^t\Longleftrightarrow t = \frac{\log n}{\log h + \log q},\\
& \quad\quad\quad L = ht\Longleftrightarrow  L =  \frac{h \log n}{\log h + \log q}\\
& \quad\quad\quad k \ge 4h(\log h + \log q + 2\log ht)
\end{split}
\end{equation}

\paragraph{Example Choice of Parameters for LPN.} The running time of our reduction is \linebreak $\poly(n,m,h,k) = \poly(n,m).$
In order to obtain hardness results, we need to ensure that this $\poly(n,m)$ running time is less than the assumed hardness of the initial $L$-dimensional noisy linear equation problem.
We formally choose the parameters in \cref{sec:parameters} but here we give a brief intuition about how large they are for concreteness.
For simplicity, we focus on the decision version of \lpn, i.e., $q = 2$.
We assume $2^{\Omega(L/\log L)}$ hardness of standard  \lpn{} and will derive a $n^{\Omega(\frac{k}{\log k (\log k + \log \log n)^2})}$ lower bound for the $k$-sparse decision version for suitable $k.$

Note that $t = \frac{\log n}{\log h + \log q} = \frac{\log n}{1 + \log h}.$ Hence, $L = ht = \frac{h\log n}{1 + \log h}.$ This value is clearly increasing in $h.$ Thus, we want to choose the largest $h$ possible.

Note, however that 
$k \ge 4h(\log h + \log q + \log (ht)^2)$ and $4h(\log h + \log q + \log (ht)^2) = \Theta(h(\log h + \log\log n)).$ Hence, we can choose $h$ at most $h = C\frac{k}{\log k + \log\log n}$ for some small absolute constant $C>0.$ Thus, $t = \frac{\log n}{\log h + \log q} =\Theta(\frac{\log n}{\log k}).$ 

Altogether, $L = ht = \Theta(\frac{k\log n}{\log k(\log k + \log\log n)}).$ We obtain  $$\exp\Big(\Omega\big(\frac{L}{\log L}\big)\Big) = \exp\Big(\Omega\big(\frac{k\log n}{\log k(\log k + \log\log n)^2}\big)\Big)$$ hardness.

% Sparse LPN:
% \begin{enumerate}
%     \item Sparse \lpn introduced by \cite{alekhovich03averagecasevsapproximation}
%     \item Some hardness evidence: \cite{liu17hardnesssparselpn}. Either sparse \lpn is hard or can build PKE from it.
%     \item 
%     \item \emph{Statistics:} \cite{feige02refutingkxor}, hardness of refuting random $k$-xor. And, \cite{Allen2015HowTR,barak16noisytensor,raghavendra17stronglyrefuting} refutation algorithms and SoS lower bounds.
%     \item \emph{Statistics:} \kirilc{Stefan, I think at some point of time you said something about hardness of learning halfspaces. Were you referring to the paper "Complexity theoretic limitations on learning DNF’s"?}
%     \item \emph{Crypto:} \cite{applebaum10pkcryptographyfromdifferentasssumptions} public-key crypto; Related to [NikonSeyoonVinod24] IO; Multiparty Homomorphic Secret Sharing (HSS) --- Jain, Lin et al.; Pseudorandom Correlation Generators.
    
%     \item \emph{Some variants and cousins:} 
%     \cite{dao24sparsedense} sparse-dense  \lpn.
% \end{enumerate}
% \medskip

% Sparse LWE: [A systematic Study of Sparse LWE, Aayush Jain Huijia Lin Sagnik Saha].

% \medskip

% Yet, very little known in terms of reductions. This is our main contribution.




% To formally state our result, for any $1\le m_1\le m,$ denote by $\mathcal{E}_{m_1}$ the distribution formed drawing $X\in \mathbb{Z}^m_q$ from $\mathcal{E}$ and restricting $X$ to a uniformly random subset of $m_1$ coordinates. Note that when $\mathcal{E}$ is the $m$-fold product distribution $\mathcal{F}^{\otimes m},$ then $\mathcal{E}_{m_1} = \mathcal{F}^{\otimes m_1}.$








\subsection{Reduction for Decision, Search, and Refutation}
\label{sec:reduction_for_all_three_tasks}

As before, \cref{eq:gadgeteq1,eq:gadgeteq2} are sufficient to obtain a reduction for any of the decision, search, and refutation tasks.
%Indeed, this is easiest to see for the search task.
%Assume that $y_i = b_i^\top s + e_i$ for some error term $e_i$.
%Then, on input $\{(b_i, y_i)\}_{i=1}^m$, we can compute $\{a_i\}_{i=1}^m$ as above and output $\{(a_i, y_i' \coloneqq y_i + a_i^\top z)\}$, where $z \in \mathbb{Z}_q^n$ is drawn uniformly at random (we add $a_i^\top z$ so that the secret is uniformly random).
%Note that $a_i$ has the correct distribution by \cref{eq:gadgeteq2}.
%Further, it holds that
%\[
%    y_i' = y_i + a_i^\top z = a_i^\top (Gs) +e_i + a_i^\top z= a_i^\top (Gs + z) + e_i \,,
%\]
%where $Gs + z$ is uniform over $\mathbb{Z}_q^n$.
Thus, given a search oracle we can recover $Gs + z$ and hence also $Gs$.
%Under the additional assumption that $G$ is full-rank we can then recover $s$.
%Our construction will have this property.
We already discussed this for the search task.
Recall that given $(b_i, y_i)$, our reduction outputs $(a_i, y_i' \coloneqq y_i + a_i^\top z)$, where $z$ is uniform over $\mathbb{Z}_q^n$.
Note that this implies that the ``planted'' distribution of the decision task will be mapped correctly.
Similarly, if in the original input $y_i$ and $b_i$ are independent then so will $y_i'$ and $a_i$ be since decoding $b_i$ into $a_i$ does not depend on $y_i$ and $y_i' = a_i^\top z + y_i$.
Note that for both decision and search, the reduction preserves the error of each equation.

% \stefanc{ToDo: Check if notation is consistent with preliniaries and technical sections}\kirilc{I think we need to fix notation here, but otherwise I really like this paragraph!}
Lastly, we discuss refutation. For simplicity of exposition, we focus on the \lpn{} setting here, but the same arguments apply to \lwe{} (see \cref{sec:reductionandtasks}).
% In particular, given $(A,y)$ we want to output a value $\phi \in [0,1]$ such that at most a $\phi$-fraction of the equations $(A,y)$ are satisfiable simultaneously.\footnote{We can also handle more general refutation tasks with respect to other error metrics, see~\cref{sec:tasks}.}
% % Further, with high probability $\phi$ should be small (ideally close to 1/2, since that is the tightest upper bound with high probability).
% % In the above we considered the slightly idealized setting in which every equation is decoded successfully with probability 1.
% % Note that for decision and search even only preserving a small 1/100 (or less) fraction of the samples would be sufficient.
% % For refutation, this is not sufficient, since our algorithm has to produce a correct upper bound on \emph{all} inputs.
% % An extreme case would be when the input is highly satisfiable, e.g., due to many duplicate rows, and the decoding process looses all the equations that make it highly satisfiable.
% % Luckily, we are able to construct gadget matrices and a decoding algorithm that only loose an $o(1)$-fraction of the samples.
Given $(A,y),$ we want two guarantees. For all approximately-satisfiable systems, i.e. $As\approx y$ for some $s,$ we want to output \textit{approximately satisfiable} with probability 1.
For the case when $A,y$ are drawn independently (and hence the system is far from satisfiable with high probability), we want to output \textit{strongly unsatisfiable}, with high probability.
% In the above we considered the slightly idealized setting in which every equation is decoded successfully with probability 1.

In the discussion on search and testing, we considered the slightly idealized setting in which every equation is decoded successfully. Yet, many reductions (including ours) lose samples.
Note that for decision and search even only preserving a small 1/100 (or less) fraction of the samples would be sufficient.
For refutation, this is not sufficient since our algorithm has to map approximately satisfiable inputs to approximately satisfiable outputs. Yet, consider the following extreme case. A very large $99/100$ fraction of the clauses in the input are satisfiable due to the fact that they are all the same $(a_1,y_1).$ The rest $1/100$ of instances are highly unsatisfiable. 
A decoding process which always fails on $a_1$ and succeeds on all the other samples
would lose the $99/100$ fraction of satisfiable equations and
could produce a highly unsatisfiable instance. 

Luckily, we are able to construct gadget matrices and a decoding algorithm that only lose a $o(1)$-fraction of the samples with high probability over worst-case inputs. Indeed, recall that each $b_j\in \Z_q^h$ is rejected with probability at most $O(\psi) = O((ht)^{-2})$ and, hence, $b$ is rejected with probability at most $O(t(ht)^{-2}) = o(1).$
This resolves the above-described issue. Hence, our reduction maps approximately satisfiable instances to approximately satisfiable instances and instances with $B,y$ independent to instances with $A,y$ independent. 
Thus, it also works for refutation.



\subsection{Organization of the Rest of the Paper}
In \cref{sec:background_short} we give formal definitions and summarize relevant prior work.
In \cref{sec:ourcontributions} we formally state our results.
%Then, we explain the challenges in reducing dense linear equations to sparse linear equations and overview how we overcome these challenges.
The following section \cref{sec:reductiontosparsity} contains the full reduction.
Our reduction as well as its run-time are parametrized. In \cref{sec:parameters} we describe several specific parameter instantiations which lead to hardness results for (sparse) \klpn{} and \klwe{} based on popular assumptions for the hardness of standard \lpn{} and  \lwe{.
We end with our application to noisy tensor completion in \cref{sec:tensorcompletion}.



% \paragraph{LPN:}
% One of the most popular instances of random noisy linear equations over finite fields is the binary case of $q = 2.$ Under certain distributional assumptions (to be described shortly), no known algorithm takes time less than $\exp(\Omega(n/\log n)),$ suggesting extremely strong hardness. 
% % When $a_1, a_2, \ldots, a_m,s\iidsim\unif(\{0,1\}^n)$ and $e_1, e_2, \ldots, e_m\iidsim \Bernoulli(1/2 - \gamma),$ this problem is known as \emph{Standard Learning Parity of Noise} (Standard \lpn). The best known algorithm for this time takes time  \cite{BKW} and there is an $\exp(\Omega(n))$ lower bound in the SQ model \cite{kearns98sq}, suggesting a near-exponential hardness of the problem. 
% % The hardness of \lpn has proven extremely useful to theoreticians. 
% From the \lpn assumption, one can construct one-way functions, secret key identification schemes \cite{krzysztof12cryptoLPN}, bit commitment schemes \cite{abhishek12comitments} and many others (see \cite{krzysztof12cryptoLPN} for more applications to cryptography). In learning theory, \lpn takes a central role in understaidng the limitations of the statistical-query model \cite{kearns98sq,BKW}  and has found applications to lower-bound constructions for
% learning probabilistic finite automata with an evaluator \cite{kearns94learnability}, certain classes of graphical models \cite{mossel06phylogeny,bresler19bolzmann} and many others.

% \paragraph{LWE:}
% Another common instance is the case of Learning With Errors (LWE) when the modulus $q$ is ``large,'' typically at least polynomial in $n$ \cite{regev05LWE}. 
% % In Standard LWE,  $a_1, a_2, \ldots, a_m,s\iidsim\unif(\mathbb{Z}_q^n)$ and $e_1, e_2, \ldots, e_m$ are independently sampled from a discrete Gaussian distribution. 
% The learning with errors problem has revolutionized cryptography, with applications to fully homomorphic encryption \cite{brakerski11fhe}, non-interactive zero-knowledge proofs \cite{canetti19fiatshamir}, public-key encryption \cite{regev05LWE}, and succinct non-interactive argument systems \cite{jin24snarg} (see \cite{peikert16decade} for more applications to cryptography). More recently, the hardness of \lwe has been used to show hardness of various statistical problems such as learning Gaussian mixture models \cite{bruna21clwe,gupte2022continuous}, learning (intersections of) halfspaces \cite{klivans06cryptographic,tiegel23agnostic,tiegel24intersection}, learning periodic neurons \cite{zadik24neurons}, and others. What makes hardness of statistical problems based on \lwe prticularly appealing is that even though \lwe is an average-case problem, under certain distributional assumptions on $A, s, e,$ it inherits a worst-case hardness from standard lattice problems \cite{regev05LWE,peikert09publickey}.

